Space-time deep neural network approximations for high-dimensional partial differential equations

It is one of the most challenging issues in applied mathematics to approximately solve high-dimensional partial differential equations (PDEs) and most of the numerical approximation methods for PDEs in the scientific literature suffer from the so-called curse of dimensionality in the sense that the number of computational operations employed in the corresponding approximation scheme to obtain an approximation precision $\varepsilon>0$ grows exponentially in the PDE dimension and/or the reciprocal of $\varepsilon$. Recently, certain deep learning based approximation methods for PDEs have been proposed and various numerical simulations for such methods suggest that deep neural network (DNN) approximations might have the capacity to indeed overcome the curse of dimensionality in the sense that the number of real parameters used to describe the approximating DNNs grows at most polynomially in both the PDE dimension $d\in\mathbb{N}$ and the reciprocal of the prescribed accuracy $\varepsilon>0$. There are now also a few rigorous results in the scientific literature which substantiate this conjecture by proving that DNNs overcome the curse of dimensionality in approximating solutions of PDEs. Each of these results establishes that DNNs overcome the curse of dimensionality in approximating suitable PDE solutions at a fixed time point $T>0$ and on a compact cube $[a,b]^d$ in space but none of these results provides an answer to the question whether the entire PDE solution on $[0,T]\times [a,b]^d$ can be approximated by DNNs without the curse of dimensionality. It is precisely the subject of this article to overcome this issue. More specifically, the main result of this work in particular proves for every $a\in\mathbb{R}$, $ b\in (a,\infty)$ that solutions of certain Kolmogorov PDEs can be approximated by DNNs on the space-time region $[0,T]\times [a,b]^d$ without the curse of dimensionality.

==> DNNapproximation.tex <==
%\textbf{TODO: Introduce ANNs instead of functions in the following Proposition!!}


\subsection{ANN approximation of the Monte Carlo Euler scheme}
\textbf{Comment: The next Proposition is a copy of Corollary 3.10 from ANN calculus paper}


\begin{prop}\label{Cor:ApproxOfMCsum}
	Let $M,N, d,\mathfrak{d} \in \N$, $\mathfrak{C},\alpha\in[0,\infty)$, $q\in(2,\infty)$,
	$a\in C(\R,\R)$ satisfy for all  $x\in \R$ that $\activation(x)=\max\{x,0\}$,
	for all $k\in\N$ let 
	$
	\left\| \cdot \right\|_{\R^k} \colon \R^k \to [0,\infty)
	$
	be the $ k $-dimensional Euclidean norm,
	let 
	$\mathbb{I}, \phi_{ 1},\phi_2\in \ANNs $
	satisfy  
	that $\dims(\mathbb{I})=(d,2d,d)$, $\inDimANN(\phi_1)=\outDimANN(\phi_1)=\inDimANN(\phi_2)=d$, and $\outDimANN(\phi_2)=\mathfrak{d}$,
	assume that for all $x,y\in\R^d$ it holds that $(\functionANN(\mathbb{I}))(x)=x$ and
	\begin{equation}\label{ApproxOfMCsum:Lipschitz}
	\left\| (\functionANN(\phi_2)) (x) - (\functionANN(\phi_2)) (y)\right\|_{\R^{\mathfrak{d}}} \leq \mathfrak{C} (1 + \left\|x\right\|_{\R^d}^{\alpha} + \left\|y \right\|_{\R^d}^{\alpha})\left\|x-y\right\|_{\R^d},
	\end{equation}
	let $p_\varepsilon\in\R$, $\varepsilon\in (0,1]$, satisfy for all $\varepsilon\in (0,1]$ that 
	\begin{equation}
	p_\varepsilon=2 \Big(\tfrac{360q}{q-2}\log_2(\eps^{-1})+\tfrac{360q}{q-2}\log_2(2^{q-1}+1)+108\Big),
	\end{equation}
	let $ ( \Omega, \mathcal{F}, \P ) $ be a probability space,
	let $X^{n,m}\colon \Omega\to \R^d$, $n\in\{0,1,\dots N-1\}$, $m\in\{1,2,\dots,M\}$, be random variables, 
	let 
	$Y^m= \big(Y^{m,x }_t(\omega)\big)_{t\in [0,T],x\in\R^d,\omega\in\Omega} \colon\allowbreak [0,T]\times \R^d\times\Omega \to \R^d $, $m\in\{1,2,\dots,M\}$, 
	%	be $ \mathcal{B}( [0,T]\times \R^d ) $/$ \mathcal{B}( \R^d ) $-measurable
	be functions 	
	which satisfy for all 
	%$ N\in\N\cap [T,\infty) $,
	$m\in\{1,2,\dots,M\}$,
	$ x \in \R^d $,
	$n\in\{0,1,\dots,N-1\}$,
	$ t \in \big[\tfrac{nT}{N},\tfrac{(n+1)T}{N}\big]$,
	$\omega\in\Omega$  
	%	that $\affineProcess^{m,x }_0(\omega)=(\functionANN(\mathbb{I}))(x)$ and
	that $\affineProcess^{m,x }_0(\omega)=x$ and
	\begin{equation}
	\label{eq:Y_processes}
	\begin{split}
	&\affineProcess^{m,x }_t(\omega) 
	=
	\affineProcess^{m,x }_{\frac{nT}{N}}(\omega)+ \left(\tfrac{tN}{T}-n\right)\left[\tfrac{T}{N}(\functionANN(\phi_{ 1 })) \big( 
	\affineProcess^{m,x }_{\frac{nT}{N}} (\omega)
	\big)
	+
	X^{n,m}(\omega)\right]
	\end{split}
	\end{equation}
%	(cf.\ Definition~\ref{Def:ANN} and Definition~\ref{Definition:ANNrealization}).
(cf.\ \textbf{TODO: Correctly cite Definitions from other paper}).
	%	Then there exists $\Psi\in \ANNs$ such that for all $t\in [0,T]$, $x \in \R^d$ it holds that
	%	$\functionANN(\Psi) \in C(\R^{d+1}, \R^{\mathfrak{d}})$
	%	and 
	%	\begin{equation}\label{ApproxOfMCsum:Estimate}
	%	 \begin{split}
	%&\left\|(\functionANN\Phi)(t,x)-\tfrac{1}{M}\left[\smallsum\limits_{m=1}^M (\functionANN(\phi_2))(Y_t^{m,x})\right]\right\|_{\R^{\mathfrak{d}}} 
	%\\&\le \tfrac{2\varepsilon {d}^{\nicefrac{1}{2}}\mathfrak{C}}{M}\left[\smallsum\limits_{m=1}^M   \left(1 + \left[6 {d}^{\nicefrac{1}{2}}
	%\sum\limits_{k=0}^N   \big(1+\left\| Y_{\frac{nT}{N}}^{m,x}\right\|_{\R^d}^2\!\big)\right]^{\alpha} + \left\|Y_t^{m,x} \right\|_{\R^d}^{\alpha}\right)	 	 	 
	%\left[\sum\limits_{n=0}^N   \big(1+\left\| Y_{t_n}^{m,x}\right\|_{\R^d}^q\!\big)\right] \right]\!.
	%\end{split}
	%	\end{equation}
	Then there exists $(\Psi_{\varepsilon,\omega})_{\varepsilon\in(0,1],\omega\in\Omega}\subseteq \ANNs$ 
	which satisfies
	\begin{enumerate}[(i)]
		\item \label{ApproxOfMCsum:ItemMeasurability}
		that for all $\varepsilon\in (0,1]$, $t\in[0,T]$, $x\in\R^d$ it holds that $\omega\ni \Omega\mapsto (\functionANN (\Psi_{\varepsilon,\omega}))(t,x)\allowbreak\in\R^{\mathfrak{d}}$ is $ \mathcal{F}$/$ \mathcal{B}( \R^{\mathfrak{d}} ) $-measurable,
		\item  that for all $\varepsilon\in(0,1]$, $\omega\in\Omega$ it holds that 	$\functionANN (\Psi_{\varepsilon,\omega})\in C(\R^{d+1},\R^{\mathfrak{d}})$,
		\item  that for all $\varepsilon\in(0,1]$, $\omega\in\Omega$,	 $n\in\{0,1,\dots, N-1\}$, $t\in [\tfrac{nT}{N},\tfrac{(n+1)T}{N}]$, $x\in\R^d$ it holds that 
		\begin{equation}
		\begin{split}
		&\left\|(\functionANN(\Psi_{\varepsilon,\omega}))(t,x)-\tfrac{1}{M}\left[\smallsum\limits_{m=1}^M (\functionANN(\phi_2))(Y_t^{m,x}(\omega))\right]\right\|_{\R^{\mathfrak{d}}} 
		\\&\le \tfrac{4\varepsilon {d}^{\nicefrac{1}{2}}\mathfrak{C}}{M}\bigg[\smallsum\limits_{m=1}^M   \left[1 + 12^\alpha {d}^{\nicefrac{\alpha}{2}}
		\Big(1+\big\| Y_{\frac{nT}{N}}^{m,x}(\omega)\big\|^2+\big\| Y_{\frac{(n+1)T}{N}}^{m,x}(\omega)\big\|^2\Big)^{\!\alpha} + \left\|Y_t^{m,x}(\omega) \right\|_{\R^d}^{\alpha}\right]
		\\&\hspace{3cm}\cdot\Big(1+\big\| Y_{\frac{nT}{N}}^{m,x}(\omega)\big\|^q+\big\| Y_{\frac{(n+1)T}{N}}^{m,x}(\omega)\big\|^q\Big) \bigg],
		\end{split}
		\end{equation}
		and
		\item \label{ApproxOfMCsum:ItemParams} that for all $\varepsilon\in(0,1]$, $\omega\in\Omega$ it holds that 
		\begin{multline}
		\paramANN(\Psi_{\varepsilon,\omega})
		\\\le M^2 \bigg((2N+1)
		\Big[d^2 p_\varepsilon+\big(
		23
		+6N(\lengthANN(\phi_1)-1)
		+  \paramANN(\mathbb{I})+N \big[\tfrac{1}{2}\paramANN(\mathbb{I})+\paramANN(\phi_1)\big]^{\!2}\big)^{\!2}\Big]
		\\\qquad-Nd(2d+1)+(\lengthANN(\phi_1)-1) d(2d+1)N(N+1)
		\bigg)^{\!2}+2 M^2 \paramANN(\phi_2).
		\end{multline}
	\end{enumerate}
\end{prop}

%\begin{proof}[Proof of Proposition~\ref{Cor:ApproxOfMCsum}]	
%	Throughout this proof  let $\varepsilon\in (0,1]$, 
%	let $(t_n)_{n\in\{0,1,\dots,N\}}\subseteq\R$
%	satisfy 
%	for all $n\in\{0,1,\dots,N\}$ that $t_n=\tfrac{n}{N}T$,
%	%	 
%	%	 for all $n\in\{0,1,\dots,N\}$ let $t_n=\tfrac{n}{N}T$,
%	let $(\Psi_{\omega,m})_{\omega\in\Omega,m\in\{1,2,\dots, M\}}\subseteq \ANNs$ satisfy	 
%	\begin{enumerate}[(I)]
%		\item
%		that for all $m\in\{1,2,\dots, M\}$, $t\in[0,T]$, $x\in\R^d$ it holds that $\omega\ni \Omega\mapsto (\functionANN (\Psi_{\omega,m}))(t,x)\allowbreak\in\R^d$ is $ \mathcal{F}$/$ \mathcal{B}( \R^d ) $-measurable,
%		\item that for all $m\in\{1,2,\dots, M\}$, $\omega\in\Omega$ it holds that $\functionANN (\Psi_{\omega,m})\in C(\R^{d+1},\R^d)$,
%		\item 
%		that for all
%		$\omega\in\Omega$, $m\in\{1,2,\dots, M\}$, $k\in\{0,1,\dots, N-1\}$, $t\in [t_{k},t_{k+1}]$, $x\in\R^d$ it holds that 
%		\begin{equation}\label{ApproxOfMCsum:EulerEstimate}
%		\left\|(\functionANN(\Psi_{\omega,m}))(t,x)-Y_t^{m,x}(\omega)\right\|_{\R^d} \le 4\varepsilon {d}^{\nicefrac{1}{2}}
%		\left(1+\big\| Y_{t_k}^{m,x}(\omega)\big\|_{\R^d}^q+\big\| Y_{t_{k+1}}^{m,x}(\omega)\big\|_{\R^d}^q\right)\!,
%		%	 \left[\smallsum\limits_{n=0}^N   \big(1+\left\| Y_{t_n}^{m,x}(\omega)\right\|_{\R^d}^q\!\big)\right]\!,
%		\end{equation}
%		\item 
%		that for all
%		$\omega\in\Omega$, $m\in\{1,2,\dots, M\}$, $k\in\{0,1,\dots, N-1\}$, $t\in [t_{k},t_{k+1}]$, $x\in\R^d$ it holds that 			
%		\begin{equation}\label{ApproxOfMCsum:EulerEstimateGrowth}
%		\begin{split}
%		\left\| (\functionANN (\Psi_{\omega,m}))(t,x)\right\|_{\R^d}
%		&\le 12 {d}^{\nicefrac{1}{2}}
%		\left(1+\big\| Y_{t_k}^{m,x}(\omega)\big\|_{\R^d}^2+\big\| Y_{t_{k+1}}^{m,x}(\omega)\big\|_{\R^d}^2\right)\!,
%		%	 \left[\smallsum\limits_{n=0}^N   \big(1+\left\| Y_{t_n}^{m,x}(\omega)\right\|_{\R^d}^2\!\big)\right]
%		\end{split}
%		\end{equation}
%		and
%		\item that for all $m\in\{1,2,\dots, M\}$, $\omega\in\Omega$ it holds that 
%		\begin{multline}\label{ApproxOfMCsum:EulerEstimateParams}
%		\paramANN(\Psi_{\omega,m})
%		\\\le\tfrac{1}{2} \bigg((2N+1)
%		\Big[d^2 p_\varepsilon+\big(
%		23
%		+6N(\lengthANN(\phi_1)-1)
%		+  \paramANN(\mathbb{I})+N [\paramANN(\mathbb{I})+\paramANN(\phi_1)]^2\big)^{\!2}\Big]
%		\\-Nd(2d+1)+(\lengthANN(\phi_1)-1) d(2d+1)N(N+1)
%		\bigg)^{\!2}
%		\end{multline}
%	\end{enumerate}	
%	(cf.\ Proposition~\ref{Cor:ApproxOfEuler}), 
%	let $(\phi_{\omega,m})_{\omega\in\Omega,m\in\{1,2,\dots, M\}}\subseteq \ANNs$ satisfy for all $\omega\in\Omega$, $m\in\{1,2,\dots, M\}$ that $\phi_{\omega,m}=\concANN{\phi_2}{\Psi_{\omega,m}}$,
%	and let $(\phi_{\omega})_{\omega\in\Omega}\subseteq \ANNs$ satisfy for all $\omega\in\Omega$, $t\in\R$, $x\in\R^{d}$ that
%	\begin{equation}\label{ApproxOfMCsum:MCsumParams}
%	\begin{split}
%	\paramANN(\Phi_\omega)\le M^2 \paramANN(\phi_{\omega,m})\qandq
%	(\functionANN (\Phi_\omega))(t,x)=\tfrac{1}{M}\smallsum\limits_{m=1}^M (\functionANN (\phi_{\omega,m}))(t,x)
%	\end{split}
%	\end{equation}
%	(cf.\ Proposition~\ref{Lemma:SumsOfANNS}).
%	%	 
%	%	 that 
%	%	 \begin{equation}
%	%	 	\Phi=\compANN{\affineMap_1}{\big[\compANN{\paraLANN{M}{\lengthANN(\concANN{\phi_2}{\Psi_1})}\big(\concANN{\phi_2}{\Psi_1},\concANN{\phi_2}{\Psi_2},\dots, \concANN{\phi_2}{\Psi_M}\big)}{\affineMap_2}\big]}.
%	%	 \end{equation}
%	Note that \eqref{ApproxOfMCsum:MCsumParams}, Propositions~\ref{Lemma:PropertiesOfConcatenations}, the fact that $\dims(\mathbb{I})=(d,2d,d)$, and \eqref{ApproxOfMCsum:EulerEstimateParams} demonstrate that 
%	\begin{equation}\label{ApproxOfMCsum:ParamEstimate}
%	\begin{split}
%	&\paramANN(\Phi_\omega)\le M^2 \paramANN(\phi_{\omega,m})
%	\le 2 M^2 \big(\paramANN(\phi_2)+\paramANN(\Psi_{\omega,1})\big)
%	\\&\le M^2 \bigg((2N+1)
%	\Big[d^2 p_\varepsilon+\big(
%	23
%	+6N(\lengthANN(\phi_1)-1)
%	+  \paramANN(\mathbb{I})+N [\paramANN(\mathbb{I})+\paramANN(\phi_1)]^2\big)^{\!2}\Big]
%	\\&\qquad-Nd(2d+1)+(\lengthANN(\phi_1)-1) d(2d+1)N(N+1)
%	\bigg)^{\!2}+2 M^2 \paramANN(\phi_2).
%	\end{split}
%	\end{equation}
%	Moreover, observe that Propositions~\ref{Lemma:PropertiesOfConcatenations} implies that for all $\omega\in\Omega$, $t\in\R$, $x\in\R^{d}$ it holds that
%	\begin{equation}\label{ApproxOfMCsum:PhiSum}
%	\begin{split}
%	(\functionANN (\Phi_\omega))(t,x)=\tfrac{1}{M}\smallsum\limits_{m=1}^M [\functionANN (\phi_{2})]\big([\functionANN(\Psi_{\omega,m})](t,x)\big).
%	\end{split}
%	\end{equation} 
%	Next note that \eqref{ApproxOfMCsum:Lipschitz}, \eqref{ApproxOfMCsum:EulerEstimate}, and \eqref{ApproxOfMCsum:EulerEstimateGrowth} ensure that for all $\omega\in\Omega$, $m\in\{1,2,\dots, M\}$,	 $k\in\{0,1,\dots, N-1\}$, $t\in [t_{k},t_{k+1}]$, $x\in\R^d$ it holds that 
%	\begin{equation}\label{ApproxOfMCsum:FinalOne}
%	\begin{split}
%	&\norm{[\functionANN (\phi_{2})]\big([\functionANN(\Psi_{\omega,m})](t,x)\big)-[\functionANN (\phi_{2})]\big(Y_t^{m,x}(\omega)\big)}_{\R^{\mathfrak{d}}}
%	\\&\le \mathfrak{C} \big(1 + \left\|(\functionANN(\Psi_{\omega,m}))(t,x)\right\|_{\R^d}^{\alpha} + \left\|Y_t^{m,x}(\omega) \right\|_{\R^d}^{\alpha}\big)\left\|(\functionANN(\Psi_{\omega,m}))(t,x)-Y_t^{m,x}(\omega)\right\|_{\R^d}
%	\\&\le 4\varepsilon {d}^{\nicefrac{1}{2}} \mathfrak{C} \left[1 + 12^\alpha {d}^{\nicefrac{\alpha}{2}}
%	\left(1+\big\| Y_{t_k}^{m,x}(\omega)\big\|_{\R^d}^2+\big\| Y_{t_{k+1}}^{m,x}(\omega)\big\|_{\R^d}^2\right)^{\!\alpha} + \left\|Y_t^{m,x}(\omega) \right\|_{\R^d}^{\alpha}\right]
%	\\&\quad\cdot\left(1+\big\| Y_{t_k}^{m,x}(\omega)\big\|_{\R^d}^q+\big\| Y_{t_{k+1}}^{m,x}(\omega)\big\|_{\R^d}^q\right)\!.
%	\end{split}
%	\end{equation}
%	Combining this with \eqref{ApproxOfMCsum:PhiSum} shows that for all 	$\omega\in\Omega$, $k\in\{0,1,\dots, N-1\}$, $t\in [t_{k},t_{k+1}]$, $x\in\R^d$ it holds that 
%	\begin{equation}\label{ApproxOfMCsum:FinalTwo}
%	\begin{split}
%	&\left\|(\functionANN(\Phi_\omega))(t,x)-\tfrac{1}{M}\left[\smallsum\limits_{m=1}^M [\functionANN(\phi_2)](Y_t^{m,x}(\omega))\right]\right\|_{\R^{\mathfrak{d}}} 
%	\\&= \left\|\tfrac{1}{M}\left[\smallsum\limits_{m=1}^M [\functionANN (\phi_{2})]\big([\functionANN(\Psi_{\omega,m})](t,x)\big)\right]-\tfrac{1}{M}\left[\smallsum\limits_{m=1}^M [\functionANN(\phi_2)](Y_t^{m,x}(\omega))\right]\right\|_{\R^{\mathfrak{d}}}
%	\\&\le \tfrac{1}{M}\left[\smallsum\limits_{m=1}^M \left\| [\functionANN (\phi_{2})]\big([\functionANN(\Psi_{\omega,m})](t,x)\big)-[(\functionANN(\phi_2)](Y_t^{m,x}(\omega))\right\|_{\R^{\mathfrak{d}}}  \right]
%	\\&\le \tfrac{4\varepsilon {d}^{\nicefrac{1}{2}}\mathfrak{C}}{M}\bigg[\smallsum\limits_{m=1}^M   \left[1 + 12^\alpha {d}^{\nicefrac{\alpha}{2}}
%	\left(1+\big\| Y_{t_k}^{m,x}(\omega)\big\|_{\R^d}^2+\big\| Y_{t_{k+1}}^{m,x}(\omega)\big\|_{\R^d}^2\right)^{\!\alpha} + \left\|Y_t^{m,x}(\omega) \right\|_{\R^d}^{\alpha}\right]
%	\\&\hspace{3cm}\cdot\left(1+\big\| Y_{t_k}^{m,x}(\omega)\big\|_{\R^d}^q+\big\| Y_{t_{k+1}}^{m,x}(\omega)\big\|_{\R^d}^q\right) \bigg]\!.
%	\end{split}
%	\end{equation}
%	Moreover, observe that the fact that for all $m\in\{1,2,\dots, M\}$, $t\in[0,T]$, $x\in\R^d$ it holds that $\omega\ni \Omega\mapsto (\functionANN (\Psi_{\omega,m}))(t,x)\in\R^{d}$ is $ \mathcal{F}$/$ \mathcal{B}( \R^{d} ) $-measurable, 
%	the fact that $\functionANN(\phi_2)$ is continuous,
%	and \eqref{ApproxOfMCsum:PhiSum} ensure that 
%	for all $t\in[0,T]$, $x\in\R^d$ it holds that $\omega\ni \Omega\mapsto (\functionANN (\phi_{\omega}))(t,x)\in\R^{\mathfrak{d}}$ is $ \mathcal{F}$/$ \mathcal{B}( \R^{\mathfrak{d}} ) $-measurable.
%	Combining this with \eqref{ApproxOfMCsum:ParamEstimate}, \eqref{ApproxOfMCsum:FinalTwo}, and the fact that $\functionANN (\Phi_\omega)\in C(\R^{d+1},\R^{\mathfrak{d}})$
%	establishes items~\eqref{ApproxOfMCsum:ItemMeasurability}--\eqref{ApproxOfMCsum:ItemParams}.
%	The proof of Proposition~\ref{Cor:ApproxOfMCsum} is thus completed.
%\end{proof}



\subsection{Approximation error estimates for ANNs}


\begin{prop}
	\label{prop:DNNerrorEstimate}
	 Let 
	$ T, \kappa \in (0,\infty) $, $\eta \in [1, \infty)$,  $p \in [2, \infty)$,
 assume for all $x\in \R$ that $\activation(x)=\max\{x,0\}$,
	let 
	$
	A_d = ( a_{ d, i, j } )_{ (i, j) \in \{ 1, \dots, d \}^2 } $ $ \in \R^{ d \times d }
	$,
	$ d \in \N $,
	be symmetric positive semidefinite matrices, 
	for every $ d \in \N $ 
	let 
	$
	\left\| \cdot \right\|_{ \R^d } \colon \R^d \to [0,\infty)
	$
	be the Euclidean norm on $\R^d$, let $\nu_d  \colon \mathcal{B}([0,T]\times\R^d) \to [0,\infty)$, $d\in\N$, be finite measures which satisfy for all $d\in\N$ that 
	%\begin{equation}
	%	\sup_{d \in \N} \left[ d^{-\theta p}
	%	\int_{\R^d}  
	%	\|{x}\|_{\R^d}^{ p \kappa } \,
	%	\nu_{ d } (dx)\right]
	%	< 
	%	\infty
	%	,
	%\end{equation}
	%$ 
	%\int_{\R^d}  
	%\|{x}\|_{\R^d}^{ p \kappa } \,
	%\nu_{ d } (dx)
	%\le \eta d^{\theta p}
	%,$
	\begin{equation}\label{DNNerrorEstimate:MeasureAssumption}
	\left[\int_{[0,T]\times \R^d} 
\|x \|_{ \R^d }^{2p \max\{2\kappa, 3\}}
\, \nu_d (d t, d x) \right]^{\!\nicefrac{1}{p}}\leq \eta d^{\eta},
	\end{equation}
	%$ \big(\textint_{[0,T]\times \R^d} 
	%\|z \|_{ \R^d }^{p \max\{2\kappa, \kappa+1\}}
	%\, \nu_d (d(s,z)) \big)^{\!\nicefrac{1}{p}}\leq \eta d^{\eta}$,
	%$ \big(\textint_{\R^d} 
	%\|z \|_{ \R^d }^{p (2\kappa+1)}
	%\, \nu_d (dz) \big)^{\!\nicefrac{1}{p}}\leq \eta d^{\eta}$,
	let
	$ f_{0,d} \colon \R^d \to \R $, $ d \in \N $,
	and
	$ f_{ 1, d } \colon \R^d \to \R^d $,
	$ d \in \N $,
	be functions,
		let 
	$
	( \phi^{ m, d }_{ \varepsilon } )_{ 
		(m, d, \varepsilon) \in \{ 0, 1 \} \times \N \times (0,1] 
	} 
	\subseteq \mathcal{N}
	$ satisfy for all
	$ d \in \N $, 
	$ \varepsilon \in (0,1] $
	that
	$
	\mathcal{R}( \phi^{ 0, d }_{ \varepsilon } )
	\in 
	C( \R^d, \R )
	$,
	$
	\mathcal{R}( \phi^{ 1, d }_{ \varepsilon } )
	\in
	C( \R^d, \R^d )
	$, and
	 $\sum_{ m = 0 }^1
	\mathcal{P}( \phi^{ m, d }_{ \varepsilon } ) 
	\leq \kappa d^{ \kappa } \varepsilon^{ - \kappa }
	$, 
	assume for all
	$ d \in \N $, 
	$ \varepsilon \in (0,1] $, 
	$ 
	x, y \in \R^d
	$
	that 
	\begin{gather}
	\label{DNNerrorEstimate:growthPhiOne}
	%	(\mathcal{R}\phi^{2,d})(x) = x, \qquad
	\left\|
	\big[\functionANN(\phi^{ 1, d }_{ \varepsilon })\big](x)    
	\right\|_{ \R^d }	
	\leq 
	\kappa ( d^{ \kappa } + \| x \|_{ \R^d } ),
	\\ \label{DNNerrorEstimate:growthMatrix}
	|
	f_{ 0, d }( x )
	| 
	+
	\smallsum\nolimits_{ i , j = 1 }^d
	| a_{ d, i, j } |
	\leq 
	\kappa d^{ \kappa }
	( 1 + \| x \|^{ \kappa }_{ \R^d } )
	,
	\\
	\label{DNNerrorEstimate:appr:coef}\left\vert 
	f_{ 0, d }(x) 
	- 
	\big[\functionANN(\phi^{ 0, d }_{ \varepsilon })\big] (x)
	\right\vert
	+
	\left\| 
	f_{ 1, d }(x) 
	- 
	\big[\functionANN(\phi^{ 1, d }_{ \varepsilon })\big] (x)
	\right\|_{ \R^d }
	\leq 
	\varepsilon \kappa d^{ \kappa }
	(
	1 + \| x \|^{ \kappa }_{ \R^d }
	),
	\\
	\label{DNNerrorEstimate:approximationLocallyLipschitz}\left\vert \big[\functionANN(\phi^{ 0, d }_{ \varepsilon })\big] (x) - \big[\functionANN(\phi^{ 0, d }_{ \varepsilon })\big] (y)\right\vert \leq \kappa d^{\kappa} (1 + \|x\|_{\R^d}^{\kappa} + \|y \|_{\R^d}^{\kappa})\|x-y\|_{\R^d},
	\end{gather}
	%\begin{gather}
	%	\label{growthPhiOne}
	%%	(\mathcal{R}\phi^{2,d})(x) = x, \qquad
	%	\|
	%	\big[\functionANN(\phi^{ 1, d }_{ \varepsilon })\big](x)    
	%	\|_{ \R^d }	
	%	\leq 
	%	\kappa ( d^{ \kappa } + \| x \|_{ \R^d } ),
	%		\\
	%	\label{eq:appr:coef}| 
	%	f_{ 0, d }(x) 
	%	- 
	%	\big[\functionANN(\phi^{ 0, d }_{ \varepsilon })\big] (x)
	%	|
	%	+
	%	\| 
	%	f_{ 1, d }(x) 
	%	- 
	%	\big[\functionANN(\phi^{ 1, d }_{ \varepsilon })\big] (x)
	%	\|_{ \R^d }
	%	\leq 
	%	\varepsilon \kappa d^{ \kappa }
	%	(
	%	1 + \| x \|^{ \kappa }_{ \R^d }
	%	),
	%	\\
	%	\label{approximationLocallyLipschitz}| \big[\functionANN(\phi^{ 0, d }_{ \varepsilon })\big] (x) - \big[\functionANN(\phi^{ 0, d }_{ \varepsilon })\big] (y)| \leq \kappa d^{\kappa} (1 + \|x\|_{\R^d}^{\kappa} + \|y \|_{\R^d}^{\kappa})\|x-y\|_{\R^d},
	%	\\ \label{growthMatrix}
	%		|
	%	f_{ 0, d }( x )
	%	| 
	%	+
	%	\smallsum\nolimits_{ i , j = 1 }^d
	%	| a_{ d, i, j } |
	%	\leq 
	%	\kappa d^{ \kappa }
	%	( 1 + \| x \|^{ \kappa }_{ \R^d } )
	%	,
	%\end{gather}
	and $\| 
	f_{ 1, d }( x ) 
	- 
	f_{ 1, d }( y )
	\|_{ \R^d }
	\leq 
	\kappa 
	\| x - y \|_{ \R^d }$, and let $ u_d \colon [0,T] \times \R^{d} \to \R $,
	$ d \in \N $, be the unique continuous functions which satisfy for all $d \in \N$ that
	$
	\inf_{q \in (0,\infty)} \allowbreak
	\sup_{(t, x) \in [0, T] \times \R^d} \allowbreak
	\frac{ | u_d(t, x) | }{ 1 + \norm{x}_{\R^d}^q }
	\allowbreak<
	\infty
	$,
	which satisfy
	for all $ d \in \N $, $ x \in \R^d $ that
	$ u_d( 0, x ) = f_{ 0, d }( x )$,
	and which satisfy for all $ d \in \N $ 
	that
	$ u_d $ is a viscosity solution of
	\begin{equation}
	\begin{split}
	( \tfrac{ \partial }{\partial t} u_d )( t, x ) 
	& = 
	( \tfrac{ \partial }{\partial x} u_d )( t, x )
	\,
	f_{ 1, d }( x )
	+
	\sum_{ i, j = 1 }^d
	a_{ d, i, j }
	\,
	( \tfrac{ \partial^2 }{ \partial x_i \partial x_j } u_d )( t, x )
	\end{split}
	\end{equation}
	for $ ( t, x ) \in (0,T) \times \R^d $ (cf.\ Theorem~\ref{thm:feynman}).
	Then 
		there exist $(\Psi_{d,N,M,\delta})_{d,N,M\in\N,\delta\in (0,1]}\subseteq \ANNs$ and $\mathcal{C},\mathfrak{C}\in (0,\infty)$ which satisfy
		\begin{enumerate}[(i)]
			\item \label{DNNerrorEstimate:Estimate} that for all 
			$d,N,M\in\N$, $\delta\in (0,1]$
			it holds that $\functionANN(\Psi_{d,N,M,\delta})\in C(\R^{d+1},\R)$ and
			\begin{equation}
			\begin{split}
			& \left[
			\int_{[0,T]\times\R^d}
			\left\vert
			u_d(y) 
			- 
			\big[\functionANN(\Psi_{d,N,M,\delta})\big](y)
			\right\vert^p
			\,
			\nu_d (d y)
			\right]^{\!\nicefrac{1}{p}} 
			\\&\le
			\mathcal{C} \left[\max\big\{1,\nu_d([0,T]\times\R^d)\big\}\right]^{\!\nicefrac{1}{p}}
			\\&\quad\cdot \left[ \frac{d^{\kappa(\kappa+4)+\max\{\eta,\kappa(2\kappa+1)\}}}{N^{1/2}}
			+ \frac{d^{\kappa+\max\{\eta,\kappa^2\}}}{M^{1/2}}
			+\delta {d}^{\nicefrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}+\eta} \right]
			\end{split}
			\end{equation}
			and
			\item \label{DNNerrorEstimate:Params}  that for all 
			$d,N,M\in\N$, $\delta\in (0,1]$
			it holds that
			\begin{equation}
			\begin{split}
			&\paramANN(\Psi_{d,N,M,\delta})
			\le \mathfrak{C} M^2 d^{8\max\{2,\kappa\}}N^{5+4\kappa} (\max\{\log_2(\delta^{-1}),1\})^2
			.
			\end{split}
			\end{equation}
		\end{enumerate}
\end{prop}

%\begin{equation}
%\begin{split}
%\paramANN(\Phi_{\varepsilon,3})&\le d^2\Big({1080}\log_2(\eps^{-1})+1080\log_2(5)+108\Big)
%\le 1080 d^2\Big(\log_2(\eps^{-1})+3\Big)
%\end{split}
%\end{equation}
%\begin{equation}
%\begin{split}
%\lengthANN(\Phi_{\varepsilon,3})\le \max \big\{\tfrac{3}{2}\log_2(\eps^{-1})+\tfrac{3}{2}\log_2(5)+\tfrac{1}{2},2\big\}
%\le \tfrac{3}{2}\log_2(\eps^{-1})+5
%\end{split}
%\end{equation}

\begin{proof}[Proof of Proposition~\ref{prop:DNNerrorEstimate}]
Throughout this proof	
%let $ \mathcal{A}_d \in \R^{ d \times d } $, $ d \in \N $, satisfy 
%	for all $ d \in \N $ that
%	$
%	\mathcal{A}_d = \sqrt{ 2 A_d }
%	$,
	let $t_n\in\R$, ${n\in\{0,1,\dots,N\}}$,
	satisfy 
	for all $n\in\{0,1,\dots,N\}$ that $t_n=\tfrac{n}{N}T$,
	let $r_{\varepsilon,q}\in\R$, $\varepsilon\in (0,1]$, $q\in (2,\infty)$ satisfy for all $\varepsilon\in (0,1]$, $q\in (2,\infty)$ that 
	\begin{equation}
	r_{\varepsilon,q}=2 \Big(\tfrac{360q}{q-2}\log_2(\eps^{-1})+\tfrac{360q}{q-2}\log_2(2^{q-1}+1)+108\Big),
	\end{equation}
	let $ ( \Omega, \mathcal{F}, \P ) $ be a probability space, 
	let $ W^{ d, m } \colon [0,T] \times \Omega \to \R^d $, $ d, m \in \N $, 
	be independent standard Brownian motions, 
	let 
	$ \affineProcess^{ N, d, m, x } \colon [0,T] \times \Omega \to \R^d $,
	%$ N\in\N\cap [T,\infty) $,
	$ N,d, m \in \N $,
	$ x \in \R^d $,
	be stochastic processes 
	which satisfy for all 
	%$ N\in\N\cap [T,\infty) $,
	$N, d, m \in \N $,
	$ x \in \R^d $,
	$n\in\{0,1,\dots,N-1\}$,
	$ t \in [t_n,t_{n+1}]$  
	that $\affineProcess^{ N, d, m, x }_0=x$ and
	\begin{equation}
	\label{eq:Y_processes}
	\begin{split}
	&\affineProcess^{ N, d, m, x }_t 
	=
	\\&\affineProcess^{ N, d, m, x }_{t_n}+ \left(\tfrac{tN}{T}-n\right)\left[\tfrac{T}{N}\big[\functionANN(\phi^{ 1, d }_{\deltaIndex})\big] \big( 
	\affineProcess^{ N, d, m, x }_{t_n} 
	\big)
	+\sqrt{ 2 A_d }
	\big(W^{ d, m }_{t_{n+1}}-W^{ d, m }_{t_n}\big)\right]
	\!,
	\end{split}
	\end{equation}
	let $ \varpi_{ d, q } \in \R $, $ d \in \N $, $ q \in (0,\infty) $, satisfy 
	for all $ q \in (0,\infty) $, $ d \in \N $  that
	\begin{equation}\label{DNNerrorEstimateVarpi}
	\begin{split}
	\varpi_{ d, q } &= 
	\max\left\{1,\sqrt{2 \max\{1,q-1\}  \operatorname{Trace}( A_d)}\right\},
	\end{split}
	\end{equation}
	let $(\mathbb{I}_d)_{d\in\N}\subseteq\ANNs$ satisfy for all $d\in\N$, $x\in\R^d$ that $\dims(\mathbb{I}_d)=(d,2d,d)$ and  $(\functionANN(\mathbb{I}_d))(x)=x$ (cf.\ Lemma~5.4 in \cite{Salimova2018}),
let $(\Psi_{d,N,M,\delta,\omega})_{d,N,M\in\N,\delta\in (0,1],\omega\in\Omega}\subseteq \ANNs$ satisfy
\begin{enumerate}[(I)]
	\item \label{ANNisRandomVariable}
	that  for all $d,N,M\in\N$, $\delta\in (0,1]$, $t\in[0,T]$, $x\in\R^d$ it holds that $\omega\ni \Omega\mapsto (\functionANN (\Psi_{d,N,M,\delta,\omega}))(t,x)\in\R$ is $ \mathcal{F}$/$ \mathcal{B}( \R ) $-measurable,
	\item
	  that 
	  for all
	  $d,N,M\in\N$, $\delta\in (0,1]$, $\omega\in\Omega$ it holds that $\functionANN(\Psi_{d,N,M,\delta,\omega})\in C(\R^{d+1},\R)$,
	 \item  that 
	 for all
	 %$N\in\N\cap [T,\infty)$, $d,M\in\N$  
	 $d,N,M\in\N$, $\delta\in (0,1]$, $\omega\in\Omega$, $k\in\{0,1,\dots,N-1\}$, $t\in [t_k,t_{k+1}]$, $x \in \R^d$   
	 it holds that
	 \begin{equation}\label{DNNerrorEstimate:BasisEstimate}
	 \begin{split}
	 &\left\vert(\functionANN(\Psi_{d,N,M,\delta,\omega}))(t,x)-\frac{ 1 }{ M }\bigg[ 
	 \textstyle
	 \sum\limits_{ m = 1 }^{M}
	 \big[\functionANN(\phi^{ 0, d }_{\deltaIndex})\big]\big(
	 \affineProcess^{N, d, m, x }_t(\omega)
	 \big)
	 \bigg]\right\vert
	 \\&\le \frac{4\delta {d}^{\nicefrac{1}{2}}\kappa d^\kappa}{M}
	 \Bigg[\sum_{m=1}^M  \left(1+\big\| Y_{t_k}^{N, d, m, x }(\omega)\big\|_{\R^d}^3+\big\| Y_{t_{k+1}}^{N, d, m, x }(\omega)\big\|_{\R^d}^3\!\right)  	 	 
	 \\&\quad\cdot
	 \left(1 + 12^\kappa {d}^{\nicefrac{\kappa}{2}}
	 \left(1+\big\| Y_{t_k}^{N, d, m, x }(\omega)\big\|_{\R^d}^2+\big\| Y_{t_{k+1}}^{N, d, m, x }(\omega)\big\|_{\R^d}^2\!\right)^\kappa + \big\|Y_t^{N, d, m, x }(\omega) \big\|_{\R^d}^\kappa\right)\Bigg],	
	 \end{split}
	 \end{equation}
	 and
	 	\item\label{DNNerrorEstimate:ParamEstimateBasis} that for all
	 	$d,N,M\in\N$, $\delta\in (0,1]$, $\omega\in\Omega$ it holds that
%	 	\begin{multline}
%	 	\paramANN(\Psi_{d,N,M,\delta,\omega})
%	 	\\\le M^2 \bigg((2N+1)
%	 	\Big[d^2 q_\delta+\big(
%	 	23
%	 	+6N(\lengthANN(\phi^{ 1, d }_{\deltaIndex})-1)
%	 	\\+  \paramANN(\mathbb{I}_d)+N [\paramANN(\mathbb{I}_d)+\paramANN(\phi^{ 1, d }_{\deltaIndex})]^2\big)^{\!2}\Big]
%	 	\\\qquad-Nd(2d+1)+(\lengthANN(\phi^{ 1, d }_{\deltaIndex})-1) d(2d+1)N(N+1)
%	 	\bigg)^{\!2}
%	 	\\+2 M^2 \paramANN(\phi^{ 0, d }_{\deltaIndex})
%	 	\end{multline}
	 	\begin{equation}
	 		\begin{split}
	 			 	&\paramANN(\Psi_{d,N,M,\delta,\omega})
	 			 	\\&\le M^2 \bigg((2N+1)
	 			 	\Big[d^2 r_{\delta,3}+\big(
	 			 	23
	 			 	+6N(\lengthANN(\phi^{ 1, d }_{\deltaIndex})-1)
	 			 	\\&\hspace{3.5cm}+\paramANN(\mathbb{I}_d)+N \big[\tfrac{1}{2}\paramANN(\mathbb{I}_d)+\paramANN(\phi^{ 1, d }_{\deltaIndex})\big]^{\!2}\big)^{\!2}\Big]
	 			 	\\&\hspace{1cm}-Nd(2d+1)+(\lengthANN(\phi^{ 1, d }_{\deltaIndex})-1) d(2d+1)N(N+1)
	 			 	\bigg)^{\!2}
	 			 	\\&\quad+2 M^2 \paramANN(\phi^{ 0, d }_{\deltaIndex})
	 		\end{split}
	 	\end{equation}
\end{enumerate}
(cf.\ Proposition~\ref{Cor:ApproxOfMCsum} (with 
$M=M$, 
$N=N$, 
$d=d$, 
$\mathfrak{d}=1$, 
$\mathfrak{C}=\kappa d^\kappa$, 
$\alpha=\kappa$, 
$q=3$, 
$a=a$, 
$\mathbb{I}=\mathbb{I}_d$,
$\phi_1=\phi^{ 1, d }_{\deltaIndex}$,
$\phi_2=\phi^{ 0, d }_{\deltaIndex}$,
$p_\varepsilon=r_{\varepsilon,3}$,
$ ( \Omega, \mathcal{F}, \P )=( \Omega, \mathcal{F}, \P ) $,
$X^{n,m}=\sqrt{ 2 A_d }
\big(W^{ d, m }_{t_{n+1}}-W^{ d, m }_{t_n}\big)$,
$Y^{m,x}=Y^{N,d,m,x}$
in the notation of Proposition~\ref{Cor:ApproxOfMCsum})), 
%(cf.\ \textbf{TODO: Correctly cite result from other paper}). 
%Observe that
%the fact that for all $ d \in \N $, 
%$ \varepsilon \in (0,1] $
%it holds
%that
%$
%\functionANN(\phi^{ 0, d }_{ \varepsilon }) 
%\in 
%C( \R^d, \R )
%$ and 
%\eqref{DNNerrorEstimate:appr:coef} ensure for all $ d \in \N $ that $f_{0,d} \in 
%C( \R^d, \R )$. This, \eqref{DNNerrorEstimate:growthMatrix}, the hypothesis that for all $d \in \N$ it holds that the function $f_{1,d} \colon \R^d \to \R^d$ is Lipschitz continuous, and
%Theorem~\ref{thm:feynman} 
%imply that there exist unique 
%continuous functions 
%$ u_d \colon [0,T] \times \R^{d} \to \R $,
%$ d \in \N $, 
%which satisfy 
%for all $d \in \N$ that
%$
%\inf_{q \in (0,\infty)} \allowbreak
%\sup_{(t, x) \in [0, T] \times \R^d} \allowbreak
%\frac{ | u_d(t, x) | }{ 1 + \norm{x}_{\R^d}^q }
%\allowbreak<
%\infty
%$,
%which satisfy
%for all $ d \in \N $, $ x \in \R^d $ that
%$ u_d( 0, x ) = f_{ 0, d }( x )$,
%and which satisfy for all $ d \in \N $ 
%that
%$ u_d $ is a viscosity solution of
%\begin{equation}
%\begin{split}
%( \tfrac{ \partial }{\partial t} u_d )( t, x ) 
%& = 
%( \tfrac{ \partial }{\partial x} u_d )( t, x )
%\,
%f_{ 1, d }( x )
%+
%\sum_{ i, j = 1 }^d
%a_{ d, i, j }
%\,
%( \tfrac{ \partial^2 }{ \partial x_i \partial x_j } u_d )( t, x )
%\end{split}
%\end{equation}
%for $ ( t, x ) \in (0,T) \times \R^d $.
%This establishes item~\eqref{DNNerrorEstimate:ItemExistence}. 
%It thus remains to prove item~\eqref{DNNerrorEstimate:Estimate}.
let $Z_{d,N,M,\delta}\colon \Omega\to \R$, $d,N,M\in\N$, $\delta\in (0,1]$, be the functions which satisfy for all $d,N,M\in\N$, $\delta\in (0,1]$, $\omega\in\Omega$ that 
\begin{equation}\label{DNNerrorEstimate:Randomvariable}
	Z_{d,N,M,\delta}(\omega)=\int_{[0,T]\times\R^d}
	\left\vert
	u_d(y) 
	- 
	\big[\functionANN(\Psi_{d,N,M,\delta,\omega})\big](y)
	\right\vert^p
	\,
	\nu_d (d y),
\end{equation}
and let $\mathcal{C}_1,\mathcal{C}_2\in (0,\infty)$ be the real numbers which satisfy that 
\begin{equation}\label{DNNerrorEstimate:FirstConstant}
\begin{split}
\mathcal{C}_1&=2 \kappa  12^{\kappa+2}  3^{\max\{0,\kappa -1\}} \big[\big(\max\{T,1\}\big)
\big(\max\{\kappa,1\}\big)\big]^{2\max\{2\kappa,3\}} 
e^{ 2\max\{2\kappa,3\}\kappa T }
\\&\quad\cdot 3^{\max\{0,2\max\{2\kappa,3\}-1\}} \left[2+(2 \max\{1,2p\max\{2\kappa,3\}-1\})^{\max\{2\kappa,3\}}\right]
\end{split}
\end{equation}
and
\begin{equation}
	\mathcal{C}_2=(\max\{1,T^{-4\kappa}\})\bigg[\bigg(3\cdot
	\Big[8640+\big(
	23
	+6\kappa  
	+7+  [4+\kappa  ]^2\big)^{\!2}\Big]
	+6\kappa  
	\bigg)^{\!2}+2\kappa\bigg].
\end{equation}
Note that for all $K\in\N$, $ z_1,z_2,\dots, z_K \in \R$, $\alpha \in (0, \infty)$ it holds that
\begin{equation}\label{DNNerrorEstimate:powerOfSums}
\left\vert\smallsum_{k=1}^K z_k\right\vert^{\alpha}  \leq K^{\max\{0,\alpha -1\}}\left[\smallsum_{k=1}^K|z_k|^{\alpha}\right].
\end{equation}
This and \eqref{DNNerrorEstimate:BasisEstimate} 
ensure that for all $d,N,M\in\N$, $\delta\in (0,1]$, $\omega\in\Omega$, $k\in\{0,1,\dots,N-1\}$, $t\in [t_k,t_{k+1}]$, $x \in \R^d$   
it holds that
\begin{equation}
\begin{split}
&\left\vert(\functionANN(\Psi_{d,N,M,\delta,\omega}))(t,x)-\frac{ 1 }{ M }\bigg[ 
\textstyle
\sum\limits_{ m = 1 }^{M}
\big[\functionANN(\phi^{ 0, d }_{\deltaIndex})\big]\big(
\affineProcess^{N, d, m, x }_t(\omega)
\big)
\bigg]\right\vert
\\&\le \frac{4\delta {d}^{\nicefrac{1}{2}}\kappa d^\kappa }{M}
\Bigg[\sum_{m=1}^M  \left(1+\big\| Y_{t_k}^{N, d, m, x }(\omega)\big\|_{\R^d}^3+\big\| Y_{t_{k+1}}^{N, d, m, x }(\omega)\big\|_{\R^d}^3\!\right)  	 	 
\\&\quad\cdot
\left(1 + 12^\kappa {d}^{\nicefrac{\kappa}{2}} \, 3^{\max\{0,\kappa -1\}}
\left(1+\big\| Y_{t_k}^{N, d, m, x }(\omega)\big\|_{\R^d}^{2\kappa}+\big\| Y_{t_{k+1}}^{N, d, m, x }(\omega)\big\|_{\R^d}^{2\kappa}\!\right)+ \big\|Y_t^{N, d, m, x }(\omega) \big\|_{\R^d}^\kappa\right)\Bigg]
\\&\le  8\delta {d}^{\nicefrac{1}{2}}\kappa d^\kappa 12^\kappa d^{\nicefrac{\kappa}{2}} 3^{\max\{0,\kappa -1\}} \tfrac{1}{M}
\Bigg[\sum_{m=1}^M  \left(1+\big\| Y_{t_k}^{N, d, m, x }(\omega)\big\|_{\R^d}^3+\big\| Y_{t_{k+1}}^{N, d, m, x }(\omega)\big\|_{\R^d}^3\!\right)  	 	 
\\&\quad\cdot
\left(1 + \big\| Y_{t_k}^{N, d, m, x }(\omega)\big\|_{\R^d}^{2\kappa}+\big\| Y_{t_{k+1}}^{N, d, m, x }(\omega)\big\|_{\R^d}^{2\kappa}+ \big\|Y_t^{N, d, m, x }(\omega) \big\|_{\R^d}^\kappa\right)\Bigg]	
\!.
\end{split}
\end{equation}
Therefore, we obtain that for all $d,N,M\in\N$, $\delta\in (0,1]$, $\omega\in\Omega$, $k\in\{0,1,\dots,N-1\}$, $t\in [t_k,t_{k+1}]$, $x \in \R^d$   
it holds that
\begin{equation}\label{DNNerrorEstimate:BasisEstimateNicer}
\begin{split}
&\left\vert(\functionANN(\Psi_{d,N,M,\delta,\omega}))(t,x)-\frac{ 1 }{ M }\bigg[ 
\textstyle
\sum\limits_{ m = 1 }^{M}
\big[\functionANN(\phi^{ 0, d }_{\deltaIndex})\big]\big(
\affineProcess^{N, d, m, x }_t(\omega)
\big)
\bigg]\right\vert
\\&\le  8\delta {d}^{\nicefrac{1}{2}}\kappa d^\kappa 12^\kappa d^{\nicefrac{\kappa}{2}} 3^{\max\{0,\kappa -1\}} \tfrac{1}{M}
%\Bigg[\sum_{m=1}^M  \left(1+\big\| Y_{t_k}^{N, d, m, x }(\omega)\big\|_{\R^d}^3+\big\| Y_{t_{k+1}}^{N, d, m, x }(\omega)\big\|_{\R^d}^3\!\right)  	 	 
\\&\cdot \Bigg[\smallsum\limits_{m=1}^M
\left(3 + \big\| Y_{t_k}^{N, d, m, x }(\omega)\big\|_{\R^d}^{\max\{2\kappa,3\}}+\big\| Y_{t_{k+1}}^{N, d, m, x }(\omega)\big\|_{\R^d}^{\max\{2\kappa,3\}}+ \big\|Y_t^{N, d, m, x }(\omega) \big\|_{\R^d}^\kappa\right)^{\!2}\Bigg]	
\!.
\end{split}
\end{equation}
Combining this and \eqref{DNNerrorEstimate:powerOfSums} proves that
for all $d,N,M\in\N$, $\delta\in (0,1]$, $\omega\in\Omega$, $k\in\{0,1,\dots,N-1\}$, $t\in [t_k,t_{k+1}]$, $x \in \R^d$   
it holds that
\begin{equation}\label{DNNerrorEstimate:BasisEstimateEvenNicer}
\begin{split}
&\left\vert(\functionANN(\Psi_{d,N,M,\delta,\omega}))(t,x)-\frac{ 1 }{ M }\bigg[ 
\textstyle
\sum\limits_{ m = 1 }^{M}
\big[\functionANN(\phi^{ 0, d }_{\deltaIndex})\big]\big(
\affineProcess^{N, d, m, x }_t(\omega)
\big)
\bigg]\right\vert
\\&\le  8\cdot 36\delta {d}^{\nicefrac{1}{2}}\kappa d^\kappa 12^{\kappa} d^{\nicefrac{\kappa}{2}} 3^{\max\{0,\kappa -1\}} \tfrac{1}{M}
\\&\cdot\Bigg[\sum_{m=1}^M   	 	 
 \left(1 + \big\| Y_{t_k}^{N, d, m, x }(\omega)\big\|_{\R^d}^{2\max\{2\kappa,3\}}+\big\| Y_{t_{k+1}}^{N, d, m, x }(\omega)\big\|_{\R^d}^{2\max\{2\kappa,3\}}+ \big\|Y_t^{N, d, m, x }(\omega) \big\|_{\R^d}^{2\kappa}\right)\Bigg]	
\!.
\end{split}
\end{equation}
%Note that 
%	\begin{equation}
%\begin{split}
%&\big( \E\big[ \| \affineProcess_t \|^3 \big] \big)^{ \nicefrac{1}{q} }
%\leq
%\Big(
%\|x\|_{\R^d} + C T 
%+ 
%\sqrt{ 2 \max\{1,3-1\} T \operatorname{Trace}(A_d )}
%\Big)
%\,
%e^{ c T }.
%\end{split}
%\end{equation}
Moreover, note that the H\"older inequality, \eqref{DNNerrorEstimate:growthPhiOne},
item~\eqref{item:EulerIII} in Lemma~\ref{lem:Euler}, 
% (with....in the notation of Lemma~\ref{lem:Euler})
and  \eqref{DNNerrorEstimateVarpi}
show that for all 
$ r \in (0,\infty) $, 
%$ \delta \in (0,1] $,
$ d, m \in \N $,
$ x \in \R^d $,
%$Z\in\{\zigZagProcess^{ \delta, d, m, x },\affineProcess_t^{N, d, m, x }\}$,
$t\in[0,T]$,
it holds that
\begin{equation}\label{DNNerrorEstimateEulerMoments}
\begin{split}
&
\big(\E\big[ 
\| \affineProcess_t^{N, d, m, x } \|^{r}
\big]
\big)^{ \nicefrac{ 1 }{r } }
\le 
\big(
\E\big[ 
\| \affineProcess_t^{N, d, m, x } \|^{\max\{r,1\}}
\big]
\big)^{ \nicefrac{ 1 }{ \max\{r,1\} } }
\\& \leq
\Big(
\|x\|_{\R^d} + \kappa d^\kappa T 
+ 
\sqrt{2 \max\{1,\max\{1,r\}-1\} T \operatorname{Trace}(A_d)}
\Big)
\,
e^{ \kappa T }
\\& \leq
\Big(
\|x\|_{\R^d} + \kappa d^\kappa T 
+ 
\sqrt{2 \max\{1,r-1\} T  \kappa d^\kappa}
\Big)
\,
e^{ \kappa T }
\\& \leq
d^\kappa\big(\max\{T,1\}\big)
\big(\max\{\kappa,1\}\big)
\Big(
\|x\|_{\R^d} + 1  
+ 
\sqrt{2 \max\{1,r-1\}   }
\Big)
\,
e^{ \kappa T }.
%\\& =
%\Big(
%\| x \|_{ \R^d }
%+
%\kappa d^{ \kappa } T
%+ 
%\varpi_{d,\max\{r,1\}} T^{\nicefrac{1}{2}}
%\Big)
%\,
%e^{
%	\kappa T
%}.
\end{split}
\end{equation}
Hence, we obtain that
for all $d,N,M\in\N$, $m\in\{1,2,\dots, M\}$, $k\in\{0,1,\dots,N-1\}$, $t\in [0,T]$, $x \in \R^d$   
it holds that
\begin{equation}
	\begin{split}
	&\max\!\left\{\Big(\E\!\left[\big\| Y_{t_k}^{N, d, m, x }\big\|_{\R^d}^{2p\max\{2\kappa,3\}}\right]\!\Big)^{\!\nicefrac{1}{p}},
	\Big(\E\!\left[\big\| Y_{t_{k+1}}^{N, d, m, x }\big\|_{\R^d}^{2p\max\{2\kappa,3\}}\right]\!\Big)^{\!\nicefrac{1}{p}},
	\Big(\E\!\left[ \big\|Y_t^{N, d, m, x } \big\|_{\R^d}^{2p\kappa}\right]\!\Big)^{\!\nicefrac{1}{p}}
	\right\}
	\\&\le \max\!\bigg\{\Big[d^\kappa\big(\max\{T,1\}\big)
	\big(\max\{\kappa,1\}\big)
	\Big(
	\|x\|_{\R^d} + 1  
	+ 
	\sqrt{2 \max\{1,2p\max\{2\kappa,3\}-1\}   }
	\Big)
	\,
	e^{ \kappa T }\Big]^{2\max\{2\kappa,3\}},
	\\&\qquad\Big[d^\kappa\big(\max\{T,1\}\big)
	\big(\max\{\kappa,1\}\big)
	\Big(
	\|x\|_{\R^d} + 1  
	+ 
	\sqrt{2 \max\{1,2p\kappa-1\}   }
	\Big)
	\,
	e^{ \kappa T }\Big]^{2\kappa}
	\bigg\}
	\\&=\Big[d^\kappa\big(\max\{T,1\}\big)
	\big(\max\{\kappa,1\}\big)
	\Big(
	\|x\|_{\R^d} + 1  
	+ 
	\sqrt{2 \max\{1,2p\max\{2\kappa,3\}-1\}   }
	\Big)
	\,
	e^{ \kappa T }\Big]^{2\max\{2\kappa,3\}}.
	\end{split}
\end{equation}
%The fact that for all $d,N,M\in\N$, $\delta\in (0,1]$ it holds  that $\Omega\times ([0,T]\times\R^d)\ni(\omega,y)\mapsto \big[\functionANN(\Psi_{d,N,M,\delta,\omega})\big](y)\in \R$ is an
%$\big( \mathcal{F}\otimes\mathcal{B}( [0,T]\times \R^d )\big) $/$ \mathcal{B}( \R ) $-measurable function,
The triangle inequality, \eqref{ANNisRandomVariable}, and \eqref{DNNerrorEstimate:BasisEstimateEvenNicer} hence demonstrate that 
for all $d,N,M\in\N$, $\delta\in (0,1]$,  $k\in\{0,1,\dots,N-1\}$, $t\in [t_k,t_{k+1}]$, $x \in \R^d$   
it holds that
\begin{equation}\label{DNNerrorEstimate:EstimateWithExpec}
\begin{split}
&\Bigg[\int_\Omega\left\vert(\functionANN(\Psi_{d,N,M,\delta,\omega}))(t,x)-\frac{ 1 }{ M }\bigg[ 
\textstyle
\sum\limits_{ m = 1 }^{M}
\big[\functionANN(\phi^{ 0, d }_{\deltaIndex})\big]\big(
\affineProcess^{N, d, m, x }_t(\omega)
\big)
\bigg]\right\vert^p\,\P(d\omega)\Bigg]^{\!\nicefrac{1}{p}}
\\&\le  2\delta {d}^{\nicefrac{1}{2}}\kappa d^\kappa 12^{\kappa+2} d^{\nicefrac{\kappa}{2}} 3^{\max\{0,\kappa -1\}} \tfrac{1}{M}
\\&\quad\cdot\Bigg[\sum_{m=1}^M   	 	 
\Big(1 + 
\Big(\E\!\left[\big\| Y_{t_k}^{N, d, m, x }\big\|_{\R^d}^{2p\max\{2\kappa,3\}}\right]\!\Big)^{\!\nicefrac{1}{p}}+
\Big(\E\!\left[\big\| Y_{t_{k+1}}^{N, d, m, x }\big\|_{\R^d}^{2p\max\{2\kappa,3\}}\right]\!\Big)^{\!\nicefrac{1}{p}}
\\&\hspace{3cm}+ \Big(\E\!\left[ \big\|Y_t^{N, d, m, x } \big\|_{\R^d}^{2p\kappa}\right]\!\Big)^{\!\nicefrac{1}{p}}\Big)\Bigg]
\\&\le  2\delta {d}^{\nicefrac{1}{2}(3\kappa+1)}\kappa  12^{\kappa+2}  3^{\max\{0,\kappa -1\}} 
\\&\quad\cdot\bigg[  	 	 
1 + 
3\Big[d^\kappa\big(\max\{T,1\}\big)
\big(\max\{\kappa,1\}\big)
\Big(
\|x\|_{\R^d} + 1  
+ 
\sqrt{2 \max\{1,2p\max\{2\kappa,3\}-1\}   }
\Big)
\,
e^{ \kappa T }\Big]^{2\max\{2\kappa,3\}}\bigg]
\\&\le  2\delta {d}^{\nicefrac{1}{2}(3\kappa+1)}\kappa  12^{\kappa+2}  3^{\max\{1,\kappa\}}  \big[d^\kappa\big(\max\{T,1\}\big)
\big(\max\{\kappa,1\}\big)\big]^{2\max\{2\kappa,3\}} e^{ 2\max\{2\kappa,3\}\kappa T }
\\&\quad\cdot\bigg[  	 	 
1 + 
\Big(
\|x\|_{\R^d} + 1  
+ 
\sqrt{2 \max\{1,2p\max\{2\kappa,3\}-1\}   }
\Big)^{2\max\{2\kappa,3\}}
\bigg].
\end{split}
\end{equation}
This, \eqref{DNNerrorEstimate:FirstConstant}, and \eqref{DNNerrorEstimate:powerOfSums} establish that 
for all $d,N,M\in\N$, $\delta\in (0,1]$, $t\in [0,T]$, $x \in \R^d$   
it holds that
\begin{equation}\label{DNNerrorEstimate:EstimateWithExpecNicer}
\begin{split}
&\Bigg[\int_\Omega\left\vert(\functionANN(\Psi_{d,N,M,\delta,\omega}))(t,x)-\frac{ 1 }{ M }\bigg[ 
\textstyle
\sum\limits_{ m = 1 }^{M}
\big[\functionANN(\phi^{ 0, d }_{\deltaIndex})\big]\big(
\affineProcess^{N, d, m, x }_t(\omega)
\big)
\bigg]\right\vert^p\,\P(d\omega)\Bigg]^{\!\nicefrac{1}{p}}
\\&\le 2\delta {d}^{\nicefrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}}\kappa  12^{\kappa+2}  3^{\max\{1,\kappa\}} \big[\big(\max\{T,1\}\big)
\big(\max\{\kappa,1\}\big)\big]^{2\max\{2\kappa,3\}} 
\\&\quad\cdot e^{ 2\max\{2\kappa,3\}\kappa T }
3^{\max\{0,2\max\{2\kappa,3\}-1\}}
\\&\quad\cdot\bigg[  	 	 
2 + 
\|x\|_{\R^d}^{2\max\{2\kappa,3\}}  
+ 
(2 \max\{1,2p\max\{2\kappa,3\}-1\})^{\max\{2\kappa,3\}}
\bigg]
\\&\le 2\delta {d}^{\nicefrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}}\kappa  12^{\kappa+2}  3^{\max\{1,\kappa\}} \big[\big(\max\{T,1\}\big)
\big(\max\{\kappa,1\}\big)\big]^{2\max\{2\kappa,3\}} 
\\&\quad\cdot e^{ 2\max\{2\kappa,3\}\kappa T }
3^{\max\{0,2\max\{2\kappa,3\}-1\}} \left[2+(2 \max\{1,2p\max\{2\kappa,3\}-1\})^{\max\{2\kappa,3\}}\right]
\\&\quad\cdot\left(1 + 
\|x\|_{\R^d}^{2\max\{2\kappa,3\}} \right) 
\\&= \delta {d}^{\nicefrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}} \mathcal{C}_1\left(1 + 
\|x\|_{\R^d}^{2\max\{2\kappa,3\}} \right) 	 	 
.
\end{split}
\end{equation}
Observe that the fact that for all $d,N,M\in\N$, $\delta\in (0,1]$, $\omega\in\Omega$ it holds that 
$\functionANN(\Psi_{d,N,M,\delta,\omega})\in C(\R^{d+1},\R)$,
the fact that for all $d,N,M\in\N$, $\delta\in (0,1]$, $t\in[0,T]$, $x\in\R^d$ it holds that $\omega\ni \Omega\mapsto (\functionANN (\Psi_{d,N,M,\delta,\omega})(t,x)\in\R$ is $ \mathcal{F}$/$ \mathcal{B}( \R ) $-measurable and Beck et al.~\cite[Lemma~2.4]{Kolmogorov} demonstrate that for all $d,N,M\in\N$, $\delta\in (0,1]$ it holds  that $\Omega\times ([0,T]\times\R^{d})\ni(\omega,y)\mapsto \big[\functionANN(\Psi_{d,N,M,\delta,\omega})\big](y)\in \R$ is 
$\big( \mathcal{F}\otimes\mathcal{B}( [0,T]\times \R^d )\big) $/$ \mathcal{B}( \R ) $-measurable.
Combining this with 
the Fubini theorem, the triangle inequality, \eqref{DNNerrorEstimate:MeasureAssumption}, and \eqref{DNNerrorEstimate:EstimateWithExpecNicer} demonstrate that for all $d,N,M\in\N$, $\delta\in (0,1]$
it holds that
\begin{equation}\label{DNNerrorEstimate:EstimateIntegratedNicer}
\begin{split}
&\Bigg[\int_\Omega \int_{ [0,T]\times\R^d }\left\vert(\functionANN(\Psi_{d,N,M,\delta,\omega}))(t,x)-\frac{ 1 }{ M }\bigg[ 
\textstyle
\sum\limits_{ m = 1 }^{M}
\big[\functionANN(\phi^{ 0, d }_{\deltaIndex})\big]\big(
\affineProcess^{N, d, m, x }_t(\omega)
\big)
\bigg]\right\vert^p\,
\\&\hspace{11.8cm}\nu_d (d t, d x) \P(d\omega)\Bigg]^{\!\nicefrac{1}{p}}
\\&\le \delta {d}^{\nicefrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}} \mathcal{C}_1
\left[\int_{ [0,T]\times\R^d}\left(1 + \|x\|_{\R^d}^{2\max\{2\kappa,3\}} \right)^p \,
	\nu_d (d t, d x)\right]^{\!\nicefrac{1}{p}}	 
\\&\le \delta {d}^{\nicefrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}} \mathcal{C}_1
\left(\eta d^\eta 
+\left[\nu_d([0,T]\times\R^d)\right]^{\!\nicefrac{1}{p}}	\right)	 
\\&\le \delta {d}^{\nicefrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}+\eta} \mathcal{C}_1 2 \eta
\left[\max\big\{1,\nu_d([0,T]\times\R^d)\big\}\right]^{\!\nicefrac{1}{p}}\!.
\end{split}
\end{equation}
%\begin{multline}\label{DNNerrorEstimate:EstimateIntegratedNicer}
%\Bigg[\int_\Omega \int_{ [0,T]\times\R^d }\left\vert(\functionANN(\Psi_{d,N,M,\delta,\omega}))(t,x)-\frac{ 1 }{ M }\bigg[ 
%\textstyle
%\sum\limits_{ m = 1 }^{M}
%\big[\functionANN(\phi^{ 0, d }_{\deltaIndex})\big]\big(
%\affineProcess^{N, d, m, x }_t(\omega)
%\big)
%\bigg]\right\vert^p\,
%\nu_d (d t, d x) \P(d\omega)\Bigg]^{\!\nicefrac{1}{p}}
%\\\le \delta {d}^{\nicefrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}} \mathcal{C}_1
%\left[\int_{ [0,T]\times\R^d}\left(1 + \|x\|_{\R^d}^{2\max\{2\kappa,3\}} \right)^p \,
%\nu_d (d t, d x)\right]^{\!\nicefrac{1}{p}}	 
%\\\le \delta {d}^{\nicefrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}} \mathcal{C}_1
%\left(\eta d^\eta 
%+\left[\nu_d([0,T]\times\R^d)\right]^{\!\nicefrac{1}{p}}	\right)	 
%\\\le \delta {d}^{\nicefrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}+\eta} \mathcal{C}_1 2 \eta
%\left[\max\big\{1,\nu_d([0,T]\times\R^d)\big\}\right]^{\!\nicefrac{1}{p}}\!.
%\end{multline}
Next note that item~\eqref{item:PDE_approxMainStatement} in Proposition~\ref{prop:PDE_approx_Lp} ensures that 
		there exists  $\mathcal{C}_2\in (0,\infty)$ which satisfies that for all 
%$N\in\N\cap [T,\infty)$, $d,M\in\N$  
$d,N,M\in\N$
it holds that 
\begin{equation}
\begin{split}
& \left(
\E\Bigg[\int_{[0,T]\times\R^d}
\bigg|
u_d(t,x) 
- 
\frac{ 1 }{ M } 
\bigg[ 
\textstyle
\sum\limits_{ m = 1 }^{M}
\big[\functionANN(\phi^{ 0, d }_{\deltaIndex})\big]\big(
\affineProcess^{N, d, m, x }_t
\big)
\bigg]
\bigg|^p
\,
\nu_d (d t, d x)
\Bigg]
\right)^{\!\nicefrac{1}{p}} 
\\&\le 
\mathcal{C}_2
%\left[N^{-\nicefrac{1}{2}}\, d^{\kappa(\kappa+4)+\max\{\eta,\kappa(2\kappa+1)\}}
% +M^{-\nicefrac{1}{2}}\, d^{\kappa+\max\{\eta,\kappa^2\}} \right]
\left[ \frac{d^{\kappa(\kappa+4)+\max\{\eta,\kappa(2\kappa+1)\}}}{N^{1/2}}
+ \frac{d^{\kappa+\max\{\eta,\kappa^2\}}}{M^{1/2}} \right] \left[\max\big\{1,\nu_d([0,T]\times\R^d)\big\}\right]^{\!\nicefrac{1}{p}}\!.
\end{split}
\end{equation}
The triangle inequality and \eqref{DNNerrorEstimate:EstimateIntegratedNicer} therefore establish that for all $d,N,M\in\N$, $\delta\in (0,1]$
it holds that
\begin{equation}
\begin{split}
&\Bigg[\int_\Omega \int_{ [0,T]\times\R^d }\left\vert u_d(y)-(\functionANN(\Psi_{d,N,M,\delta,\omega}))(y)\right\vert^p\,
\nu_d (d y) \P(d\omega)\Bigg]^{\!\nicefrac{1}{p}}
\\&\le
\left(
\E\Bigg[\int_{[0,T]\times\R^d}
\bigg|
u_d(t,x) 
- 
\frac{ 1 }{ M } 
\bigg[ 
\textstyle
\sum\limits_{ m = 1 }^{M}
\big[\functionANN(\phi^{ 0, d }_{\deltaIndex})\big]\big(
\affineProcess^{N, d, m, x }_t
\big)
\bigg]
\bigg|^p
\,
\nu_d (d t, d x)
\Bigg]
\right)^{\!\nicefrac{1}{p}}
\\&+
\Bigg[\int_\Omega \int_{ [0,T]\times\R^d }\left\vert(\functionANN(\Psi_{d,N,M,\delta,\omega}))(t,x)-\frac{ 1 }{ M }\bigg[ 
\textstyle
\sum\limits_{ m = 1 }^{M}
\big[\functionANN(\phi^{ 0, d }_{\deltaIndex})\big]\big(
\affineProcess^{N, d, m, x }_t(\omega)
\big)
\bigg]\right\vert^p
\\&\hspace{11.8cm}\nu_d (d t, d x) \P(d\omega)\Bigg]^{\!\nicefrac{1}{p}}
\\&\le
\mathcal{C}_2
\left[ \frac{d^{\kappa(\kappa+4)+\max\{\eta,\kappa(2\kappa+1)\}}}{N^{1/2}}
+ \frac{d^{\kappa+\max\{\eta,\kappa^2\}}}{M^{1/2}} \right] \left[\max\big\{1,\nu_d([0,T]\times\R^d)\big\}\right]^{\!\nicefrac{1}{p}}
 \\&\quad+\delta {d}^{\nicefrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}+\eta} \mathcal{C}_1 2 \eta
\left[\max\big\{1,\nu_d([0,T]\times\R^d)\big\}\right]^{\!\nicefrac{1}{p}}
%\\&\le
%\max\{\mathcal{C}_2, 2\mathcal{C}_1  \eta\} \left[\max\big\{1,\nu_d([0,T]\times\R^d)\big\}\right]^{\!\nicefrac{1}{p}}
% \\&\quad\cdot \left[ \frac{d^{\kappa(\kappa+4)+\max\{\eta,\kappa(2\kappa+1)\}}}{N^{1/2}}
% + \frac{d^{\kappa+\max\{\eta,\kappa^2\}}}{M^{1/2}}
% +\delta {d}^{\nicefrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}+\eta} \right]
\!.
\end{split}
\end{equation}
Hence, we obtain that for all $d,N,M\in\N$, $\delta\in (0,1]$
it holds that
\begin{equation}
\begin{split}
&\Bigg[\int_\Omega \int_{ [0,T]\times\R^d }\left\vert u_d(y)-(\functionANN(\Psi_{d,N,M,\delta,\omega}))(y)\right\vert^p\,
\nu_d (d y) \P(d\omega)\Bigg]^{\!\nicefrac{1}{p}}
\\&\le
\max\{\mathcal{C}_2, 2\mathcal{C}_1  \eta\} \left[\max\big\{1,\nu_d([0,T]\times\R^d)\big\}\right]^{\!\nicefrac{1}{p}}
\\&\quad\cdot \left[ \frac{d^{\kappa(\kappa+4)+\max\{\eta,\kappa(2\kappa+1)\}}}{N^{1/2}}
+ \frac{d^{\kappa+\max\{\eta,\kappa^2\}}}{M^{1/2}}
+\delta {d}^{\nicefrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}+\eta} \right]
\!.
\end{split}
\end{equation}
The fact that for all $d,N,M\in\N$, $\delta\in (0,1]$ it holds  that $\Omega\times ([0,T]\times\R^d)\ni(\omega,y)\mapsto \big[\functionANN(\Psi_{d,N,M,\delta,\omega})\big](y)\in \R$ is a
$\big( \mathcal{F}\otimes\mathcal{B}( [0,T]\times \R^d )\big) $/$ \mathcal{B}( \R ) $-measurable function and \eqref{DNNerrorEstimate:Randomvariable} hence  imply that $Z_{d,N,M,\delta}\colon \Omega\to \R$, $d,N,M\in\N$, $\delta\in (0,1]$, are random variables which satisfy for all $d,N,M\in\N$, $\delta\in (0,1]$ that 
\begin{equation}
\begin{split}
\E \big[\vert Z_{d,N,M,\delta}\vert \big]&\le \left[\max\{\mathcal{C}_2, 2\mathcal{C}_1  \eta\}\right]^{p} \max\big\{1,\nu_d([0,T]\times\R^d)\big\}
\\&\quad\cdot \left[ \frac{d^{\kappa(\kappa+4)+\max\{\eta,\kappa(2\kappa+1)\}}}{N^{1/2}}
+ \frac{d^{\kappa+\max\{\eta,\kappa^2\}}}{M^{1/2}}
+\delta {d}^{\nicefrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}+\eta} \right]^p
\!.
\end{split}
\end{equation}
Grohs et al.~\cite[Proposition~3.3]{GrohsWurstemberger2018} hence proves that for all $d,N,M\in\N$, $\delta\in (0,1]$ there exists $\mathfrak{w}_{d,N,M,\delta} \in \Omega$ which satisfies that 
\begin{equation}\label{finalEstimateError}
\begin{split}
&Z_{d,N,M,\delta}(\mathfrak{w}_{d,N,M,\delta})\le \left[\max\{\mathcal{C}_2, 2\mathcal{C}_1  \eta\}\right]^{p} \max\big\{1,\nu_d([0,T]\times\R^d)\big\}
\\&\quad\cdot \left[ \frac{d^{\kappa(\kappa+4)+\max\{\eta,\kappa(2\kappa+1)\}}}{N^{1/2}}
+ \frac{d^{\kappa+\max\{\eta,\kappa^2\}}}{M^{1/2}}
+\delta {d}^{\nicefrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}+\eta} \right]^p
\!.
\end{split}
\end{equation}
In addition, note that for all $\varepsilon\in (0,1]$ it holds that 
\begin{equation}
\begin{split}
r_{\varepsilon,3}&=2 \Big(1080\log_2(\eps^{-1})+1080\log_2(5)+108\Big)
\\&\le 2 \Big(1080\log_2(\eps^{-1})+1080\cdot 3\Big)
= 2160 \Big(\log_2(\eps^{-1})+ 3\Big).
\end{split}
\end{equation}
This, the hypothesis that for all $\varepsilon\in (0,1]$, $d\in\N$, $m\in\{0,1\}$ it holds that $
\lengthANN( \phi^{ m, d }_{ \varepsilon } ) \le\mathcal{P}( \phi^{ m, d }_{ \varepsilon } ) 
\leq \kappa d^{ \kappa } \varepsilon^{ - \kappa }
$, the fact that for all $d\in\N$ it holds that $\paramANN(\mathbb{I}_d)=2d(d+1)+d(2d+1)\le 7d^2$, and \eqref{DNNerrorEstimate:ParamEstimateBasis} prove  that for all
$d,N,M\in\N$, $\delta\in (0,1]$, $\omega\in\Omega$ it holds that
\begin{equation}
\begin{split}
&\paramANN(\Psi_{d,N,M,\delta,\omega})
\\&\le M^2 \bigg((2N+1)
\Big[d^2 r_{\delta,3}+\big(
23
+6N(\lengthANN(\phi^{ 1, d }_{\deltaIndex})-1)
\\&\hspace{3.5cm}+\paramANN(\mathbb{I}_d)+N \big[\tfrac{1}{2}\paramANN(\mathbb{I}_d)+\paramANN(\phi^{ 1, d }_{\deltaIndex})\big]^{\!2}\big)^{\!2}\Big]
\\&\hspace{1cm}-Nd(2d+1)+(\lengthANN(\phi^{ 1, d }_{\deltaIndex})-1) d(2d+1)N(N+1)
\bigg)^{\!2}
\\&\quad+2 M^2 \paramANN(\phi^{ 0, d }_{\deltaIndex})
\\&\le M^2 \bigg((2N+1)
\Big[2160 d^2 \Big(\log_2(\delta^{-1})+ 3\Big)+\big(
23
+6N\kappa d^{ \kappa } (\min\{(T/N)^{  1/2},1\})^{-\kappa}
\\&\hspace{5cm}+7d^2+N [4d^2+\kappa d^{ \kappa } (\min\{(T/N)^{1/2},1\})^{-\kappa}]^2\big)^{\!2}\Big]
\\&\hspace{3cm}-Nd(2d+1)+\kappa d^{ \kappa } (\min\{(T/N)^{1/2},1\})^{-\kappa} d(2d+1)N(N+1)
\bigg)^{\!2}
\\&\quad+2 M^2 \kappa d^{ \kappa } (\min\{(T/N)^{1/2},1\})^{-\kappa}.
\end{split}
\end{equation}
Hence, we obtain that
\begin{equation}
\begin{split}
&\paramANN(\Psi_{d,N,M,\delta,\omega})
\\&\le M^2 \bigg((2N+1)
\Big[2160 d^2 \Big(\log_2(\delta^{-1})+ 3\Big)+\big(
23
+6N^{1+\kappa/2}\kappa d^{ \kappa } \max\{T^{ - \kappa/2},1\}
\\&\hspace{5cm}+7d^2+N^{1+\kappa} [4d^2+\kappa d^{ \kappa } \max\{T^{ - \kappa/2},1\}]^2\big)^{\!2}\Big]
\\&\hspace{3cm}+6\kappa d^{ 2+\kappa } \max\{T^{ - \kappa/2},1\}N^{2+\kappa/2}
\bigg)^{\!2}
\\&\quad+2\kappa M^2 N^{\kappa/2}  d^{ \kappa } \max\{T^{ - \kappa/2},1\}.
\end{split}
\end{equation}
This ensures that
\begin{equation}
\begin{split}
&\paramANN(\Psi_{d,N,M,\delta,\omega})
\\&\le M^2 \bigg((2N+1)
\Big[2160 d^2 \Big(\log_2(\delta^{-1})+ 3\Big)
\\&\hspace{1.5cm}+N^{2(1+\kappa)}(\max\{T^{ - \kappa/2},1\})^4\big(
23
+6\kappa d^\kappa 
+7d^2+ d^{2\max\{2,\kappa\}} [4+\kappa  ]^2\big)^{\!2}\Big]
\\&\hspace{1.5cm}+6\kappa d^{ 2+\kappa } \max\{T^{ - \kappa/2},1\}N^{2+\kappa/2}
\bigg)^{\!2}
\\&\quad+2\kappa M^2 N^{\kappa/2}  d^{ \kappa } \max\{T^{ - \kappa/2},1\}.
%\\&\le M^2 \bigg(3N N^{4(1+\kappa)}
%d^{4\max\{2,\kappa\}}\Big[2160  \Big(\log_2(\delta^{-1})+ 3\Big)+\big(
%23
%+6\kappa  T^{ - \kappa/2}
%\\&\hspace{5cm}+7+ [4+\kappa  T^{ - \kappa/2}]^2\big)^{\!2}\Big]
%\\&\hspace{3cm}+6\kappa d^{ 2+\kappa } T^{ - \kappa/2}N^{2+\kappa/2}
%\bigg)^{\!2}
%\\&\quad+2\kappa M^2 N^{\kappa/2}  d^{ \kappa } T^{ - \kappa/2}
%\\&\le M^2 d^{8\max\{2,\kappa\}}N^{5+4\kappa}\bigg(
%\Big[2160  \Big(\log_2(\delta^{-1})+ 3\Big)+\big(
%23
%+6\kappa  T^{ - \kappa/2}
%\\&\hspace{5cm}+7+  [4+\kappa  T^{ - \kappa/2}]^2\big)^{\!2}\Big]
%+6\kappa  T^{ - \kappa/2}
%\bigg)^{\!2}
%\\&\quad+2\kappa M^2 N^{\kappa/2}  d^{ \kappa } T^{ - \kappa/2}.
\end{split}
\end{equation}
Therefore, we obtain that
\begin{equation}
\begin{split}
&\paramANN(\Psi_{d,N,M,\delta,\omega})
%\\&\le M^2 \bigg((2N+1)
%\Big[2160 d^2 \Big(\log_2(\delta^{-1})+ 3\Big)+N^{2(1+\kappa)}\big(
%23
%+6\kappa d^\kappa 
%\\&\hspace{5cm}+7d^2+ d^{2\max\{2,\kappa\}} [4+\kappa  ]^2\big)^{\!2}\Big]
%\\&\hspace{3cm}+6\kappa d^{ 2+\kappa } N^{2+\kappa/2}
%\bigg)^{\!2}
%\\&\quad+2\kappa M^2 N^{\kappa/2}  d^{ \kappa } 
\\&\le M^2 (\max\{T^{ - \kappa/2},1\})^8
\\&\quad\cdot\bigg(3N N^{2(1+\kappa)}
d^{4\max\{2,\kappa\}}\Big[2160  \Big(\log_2(\delta^{-1})+ 3\Big)+\big(
23
+6\kappa  
+7+ [4+\kappa  ]^2\big)^{\!2}\Big]
\\&\hspace{1cm}+6\kappa d^{ 2+\kappa } N^{2+\kappa/2}
\bigg)^{\!2}
\\&\quad+2\kappa M^2 N^{\kappa/2}  d^{ \kappa } \max\{T^{ - \kappa/2},1\}
\\&\le M^2 (\max\{T^{ - 4\kappa},1\})\, d^{8\max\{2,\kappa\}}N^{5+4\kappa}
\\&\quad\cdot\bigg(3\cdot\Big[2160  \Big(\log_2(\delta^{-1})+ 3\Big)+\big(
23+6\kappa  +7+  [4+\kappa  ]^2\big)^{\!2}\Big]
+6\kappa  
\bigg)^{\!2}
\\&\quad+2\kappa M^2 N^{\kappa/2}  d^{ \kappa } \max\{T^{ - \kappa/2},1\}.
\end{split}
\end{equation}
Hence, we obtain that 
\begin{equation}
\begin{split}
&\paramANN(\Psi_{d,N,M,\delta,\omega})
\\&\le M^2 (\max\{T^{ - 4\kappa},1\})\, d^{8\max\{2,\kappa\}}N^{5+4\kappa}
\\&\quad\cdot\bigg(
3\cdot\Big[8640  \max\{\log_2(\delta^{-1}),1\}+\big(
23
+6\kappa 
+7+  [4+\kappa  ]^2\big)^{\!2}\Big]
+6\kappa  
\bigg)^{\!2}
\\&\quad+2\kappa M^2 N^{\kappa/2}  d^{ \kappa }  \max\{T^{ - \kappa/2},1\}
\\&\le M^2 (\max\{T^{ - 4\kappa},1\})\, d^{8\max\{2,\kappa\}}N^{5+4\kappa} (\max\{\log_2(\delta^{-1}),1\})^2\\&\quad\cdot\bigg(
3\cdot\Big[8640+\big(
23
+6\kappa  
+7+  [4+\kappa  ]^2\big)^{\!2}\Big]
+6\kappa  
\bigg)^{\!2}
\\&\quad+2\kappa M^2 N^{\kappa/2}  d^{ \kappa }  \max\{T^{ - \kappa/2},1\}.
%\\&\le M^2 d^{8\max\{2,\kappa\}}N^{5+4\kappa} (\max\{1,T^{-4\kappa}\})(\max\{\log_2(\delta^{-1}),1\})\\&\quad\cdot\bigg[\bigg(
%3\cdot\Big[8640+\big(
%23
%+6\kappa  
%+7+  [4+\kappa  ]^2\big)^{\!2}\Big]
%+6\kappa  
%\bigg)^{\!2}+2\kappa\bigg]
%\\&=\mathcal{C}_2 M^2 d^{8\max\{2,\kappa\}}N^{5+4\kappa} (\max\{\log_2(\delta^{-1}),1\})
%.
\end{split}
\end{equation}
This demonstrates that 
\begin{equation}
\begin{split}
\paramANN(\Psi_{d,N,M,\delta,\omega})
%\\&\le M^2 d^{8\max\{2,\kappa\}}N^{5+4\kappa}\bigg(
%\Big[8640  \max\{\log_2(\delta^{-1}),1\}+\big(
%23
%+6\kappa  (\max\{1,T^{-\kappa}\})
%\\&\hspace{4cm}+7+ (\max\{1,T^{-\kappa}\}) [4+\kappa  ]^2\big)^{\!2}\Big]
%+6\kappa  (\max\{1,T^{-2\kappa}\})
%\bigg)^{\!2}
%\\&\quad+2\kappa M^2 N^{\kappa/2}  d^{ \kappa }  T^{ - \kappa/2}
%\\&\le M^2 d^{8\max\{2,\kappa\}}N^{5+4\kappa} (\max\{1,T^{-4\kappa}\})(\max\{\log_2(\delta^{-1}),1\})\\&\quad\cdot\bigg(
%\Big[8640+\big(
%23
%+6\kappa  
%+7+  [4+\kappa  ]^2\big)^{\!2}\Big]
%+6\kappa  
%\bigg)^{\!2}
%\\&\quad+2\kappa M^2 N^{\kappa/2}  d^{ \kappa }  T^{ - \kappa/2}
&\le M^2 (\max\{1,T^{-4\kappa}\})\, d^{8\max\{2,\kappa\}}N^{5+4\kappa}(\max\{\log_2(\delta^{-1}),1\})^2\\&\quad\cdot\bigg[\bigg(
3\cdot\Big[8640+\big(
23
+6\kappa  
+7+  [4+\kappa  ]^2\big)^{\!2}\Big]
+6\kappa  
\bigg)^{\!2}+2\kappa\bigg]
\\&=\mathcal{C}_2 M^2 d^{8\max\{2,\kappa\}}N^{5+4\kappa} (\max\{\log_2(\delta^{-1}),1\})^2
.
\end{split}
\end{equation}
Combining this, \eqref{DNNerrorEstimate:Randomvariable}, and \eqref{finalEstimateError} establishes item~\eqref{DNNerrorEstimate:Estimate} and item~\eqref{DNNerrorEstimate:Params}.
	The proof of Proposition~\ref{prop:DNNerrorEstimate} is thus completed.
\end{proof}








\subsection{Cost estimates for ANNs}





\begin{theorem}
	\label{theorem:DNNerrorEstimate}
	Let 
	$ T, \kappa \in (0,\infty) $, $\eta \in [1, \infty)$,  $p \in [2, \infty)$,
	 assume for all $x\in \R$ that $\activation(x)=\max\{x,0\}$,
	let 
	$
	A_d = ( a_{ d, i, j } )_{ (i, j) \in \{ 1, \dots, d \}^2 } $ $ \in \R^{ d \times d }
	$,
	$ d \in \N $,
	be symmetric positive semidefinite matrices, 
	for every $ d \in \N $ 
	let 
	$
	\left\| \cdot \right\|_{ \R^d } \colon \R^d \to [0,\infty)
	$
	be the Euclidean norm on $\R^d$, let $\nu_d  \colon \mathcal{B}([0,T]\times\R^d) \to [0,\infty)$, $d\in\N$, be finite measures which satisfy for all $d\in\N$ that 
	%\begin{equation}
	%	\sup_{d \in \N} \left[ d^{-\theta p}
	%	\int_{\R^d}  
	%	\|{x}\|_{\R^d}^{ p \kappa } \,
	%	\nu_{ d } (dx)\right]
	%	< 
	%	\infty
	%	,
	%\end{equation}
	%$ 
	%\int_{\R^d}  
	%\|{x}\|_{\R^d}^{ p \kappa } \,
	%\nu_{ d } (dx)
	%\le \eta d^{\theta p}
	%,$
	\begin{equation}\label{theoremDNNerrorEstimate:MeasureAssumption}
	\left[\max\!\left\{1,\nu_d([0,T]\times\R^d),\int_{[0,T]\times \R^d} 
	\|x \|_{ \R^d }^{2p \max\{2\kappa, 3\}}
	\, \nu_d (d t, d x) \right\}\right]^{\!\nicefrac{1}{p}}\leq \eta d^{\eta},
	\end{equation}
	%$ \big(\textint_{[0,T]\times \R^d} 
	%\|z \|_{ \R^d }^{p \max\{2\kappa, \kappa+1\}}
	%\, \nu_d (d(s,z)) \big)^{\!\nicefrac{1}{p}}\leq \eta d^{\eta}$,
	%$ \big(\textint_{\R^d} 
	%\|z \|_{ \R^d }^{p (2\kappa+1)}
	%\, \nu_d (dz) \big)^{\!\nicefrac{1}{p}}\leq \eta d^{\eta}$,
	let
	$ f_{0,d} \colon \R^d \to \R $, $ d \in \N $,
	and
	$ f_{ 1, d } \colon \R^d \to \R^d $,
	$ d \in \N $,
	be functions,
	let 
	$
	( \phi^{ m, d }_{ \varepsilon } )_{ 
		(m, d, \varepsilon) \in \{ 0, 1 \} \times \N \times (0,1] 
	} 
	\subseteq \mathcal{N}
	$ satisfy for all
	$ d \in \N $, 
	$ \varepsilon \in (0,1] $
	that
	$
	\mathcal{R}( \phi^{ 0, d }_{ \varepsilon } )
	\in 
	C( \R^d, \R )
	$,
	$
	\mathcal{R}( \phi^{ 1, d }_{ \varepsilon } )
	\in
	C( \R^d, \R^d )
	$, and
	$\sum_{ m = 0 }^1
	\mathcal{P}( \phi^{ m, d }_{ \varepsilon } ) 
	\leq \kappa d^{ \kappa } \varepsilon^{ - \kappa }
	$,  
	assume for all
	$ d \in \N $, 
	$ \varepsilon \in (0,1] $, 
	$ 
	x, y \in \R^d
	$
	that 
	\begin{gather}
	\label{theoremDNNerrorEstimate:growthPhiOne}
	%	(\mathcal{R}\phi^{2,d})(x) = x, \qquad
	\|
	\big[\functionANN(\phi^{ 1, d }_{ \varepsilon })\big](x)    
	\|_{ \R^d }	
	\leq 
	\kappa ( d^{ \kappa } + \| x \|_{ \R^d } ),
	\\ \label{theoremDNNerrorEstimate:growthMatrix}
	|
	f_{ 0, d }( x )
	| 
	+
	\smallsum\nolimits_{ i , j = 1 }^d
	| a_{ d, i, j } |
	\leq 
	\kappa d^{ \kappa }
	( 1 + \| x \|^{ \kappa }_{ \R^d } )
	,
	\\
	\label{theoremDNNerrorEstimate:appr:coef}| 
	f_{ 0, d }(x) 
	- 
	\big[\functionANN(\phi^{ 0, d }_{ \varepsilon })\big] (x)
	|
	+
	\| 
	f_{ 1, d }(x) 
	- 
	\big[\functionANN(\phi^{ 1, d }_{ \varepsilon })\big] (x)
	\|_{ \R^d }
	\leq 
	\varepsilon \kappa d^{ \kappa }
	(
	1 + \| x \|^{ \kappa }_{ \R^d }
	),
	\\
	\label{theoremDNNerrorEstimate:approximationLocallyLipschitz}| \big[\functionANN(\phi^{ 0, d }_{ \varepsilon })\big] (x) - \big[\functionANN(\phi^{ 0, d }_{ \varepsilon })\big] (y)| \leq \kappa d^{\kappa} (1 + \|x\|_{\R^d}^{\kappa} + \|y \|_{\R^d}^{\kappa})\|x-y\|_{\R^d},
	\end{gather}
	%\begin{gather}
	%	\label{growthPhiOne}
	%%	(\mathcal{R}\phi^{2,d})(x) = x, \qquad
	%	\|
	%	\big[\functionANN(\phi^{ 1, d }_{ \varepsilon })\big](x)    
	%	\|_{ \R^d }	
	%	\leq 
	%	\kappa ( d^{ \kappa } + \| x \|_{ \R^d } ),
	%		\\
	%	\label{eq:appr:coef}| 
	%	f_{ 0, d }(x) 
	%	- 
	%	\big[\functionANN(\phi^{ 0, d }_{ \varepsilon })\big] (x)
	%	|
	%	+
	%	\| 
	%	f_{ 1, d }(x) 
	%	- 
	%	\big[\functionANN(\phi^{ 1, d }_{ \varepsilon })\big] (x)
	%	\|_{ \R^d }
	%	\leq 
	%	\varepsilon \kappa d^{ \kappa }
	%	(
	%	1 + \| x \|^{ \kappa }_{ \R^d }
	%	),
	%	\\
	%	\label{approximationLocallyLipschitz}| \big[\functionANN(\phi^{ 0, d }_{ \varepsilon })\big] (x) - \big[\functionANN(\phi^{ 0, d }_{ \varepsilon })\big] (y)| \leq \kappa d^{\kappa} (1 + \|x\|_{\R^d}^{\kappa} + \|y \|_{\R^d}^{\kappa})\|x-y\|_{\R^d},
	%	\\ \label{growthMatrix}
	%		|
	%	f_{ 0, d }( x )
	%	| 
	%	+
	%	\smallsum\nolimits_{ i , j = 1 }^d
	%	| a_{ d, i, j } |
	%	\leq 
	%	\kappa d^{ \kappa }
	%	( 1 + \| x \|^{ \kappa }_{ \R^d } )
	%	,
	%\end{gather}
	and $\| 
	f_{ 1, d }( x ) 
	- 
	f_{ 1, d }( y )
	\|_{ \R^d }
	\leq 
	\kappa 
	\| x - y \|_{ \R^d }$, 
	and let $ u_d \colon [0,T] \times \R^{d} \to \R $,
	$ d \in \N $, be the unique continuous functions which satisfy for all $d \in \N$ that
	$
	\inf_{q \in (0,\infty)} \allowbreak
	\sup_{(t, x) \in [0, T] \times \R^d} \allowbreak
	\frac{ | u_d(t, x) | }{ 1 + \norm{x}_{\R^d}^q }
	\allowbreak<
	\infty
	$,
	which satisfy
	for all $ d \in \N $, $ x \in \R^d $ that
	$ u_d( 0, x ) = f_{ 0, d }( x )$,
	and which satisfy for all $ d \in \N $ 
	that
	$ u_d $ is a viscosity solution of
	\begin{equation}
	\begin{split}
	( \tfrac{ \partial }{\partial t} u_d )( t, x ) 
	& = 
	( \tfrac{ \partial }{\partial x} u_d )( t, x )
	\,
	f_{ 1, d }( x )
	+
	\sum_{ i, j = 1 }^d
	a_{ d, i, j }
	\,
	( \tfrac{ \partial^2 }{ \partial x_i \partial x_j } u_d )( t, x )
	\end{split}
	\end{equation}
	for $ ( t, x ) \in (0,T) \times \R^d $ (cf.\ Theorem~\ref{thm:feynman}).
	Then there exist $\mathcal{C}\in (0,\infty)$ and $(\Psi_{d,\varepsilon})_{d\in\N,\varepsilon\in (0,1]}\subseteq \ANNs$ which satisfy
	\begin{enumerate}[(i)]
		\item
		\label{theoremDNNerrorEstimate:Estimate}
		 that for all 
		%$N\in\N\cap [T,\infty)$, $d,M\in\N$  
		$d\in\N$, $\varepsilon\in (0,1]$
		it holds that $\functionANN(\Psi_{d,\varepsilon})\in C(\R^{d+1},\R)$ and
		\begin{equation}
		\begin{split}
		& \left[
		\int_{[0,T]\times\R^d}
		\left\vert
		u_d(y) 
		- 
		\big[\functionANN(\Psi_{d,\varepsilon})\big](y)
		\right\vert^p
		\,
		\nu_d (d y)
		\right]^{\!\nicefrac{1}{p}} 
		\le
		\varepsilon
		\end{split}
		\end{equation}
		and
		\item \label{theoremDNNerrorEstimate:Param}
		that for all 
		$d\in\N$, $\varepsilon\in (0,1]$
		it holds that
		 \begin{equation}
		\begin{split}
		&\paramANN(\Psi_{d,\varepsilon})
		\\&\le \mathcal{C} \varepsilon^{-16-8\kappa}  d^{2+4\kappa+4\max\{\eta,\kappa^2\}+4\eta+8\max\{2,\kappa\}+[2\kappa(\kappa+4)+2\max\{\eta,\kappa(2\kappa+1)\}+2\eta](5+4\kappa)}. 
		\end{split}
		\end{equation}
	\end{enumerate}
\end{theorem}

\begin{proof}[Proof of Theorem~\ref{theorem:DNNerrorEstimate}]
%	Observe that item~\eqref{DNNerrorEstimate:ItemExistence} in Proposition~\ref{prop:DNNerrorEstimate} ensures that 
%	there exist unique 
%	continuous functions 
%	$ u_d \colon [0,T] \times \R^{d} \to \R $,
%	$ d \in \N $, 
%	which satisfy 
%	for all $d \in \N$ that
%	$
%	\inf_{q \in (0,\infty)} \allowbreak
%	\sup_{(t, x) \in [0, T] \times \R^d} \allowbreak
%	\frac{ | u_d(t, x) | }{ 1 + \norm{x}_{\R^d}^q }
%	\allowbreak<
%	\infty
%	$,
%	which satisfy
%	for all $ d \in \N $, $ x \in \R^d $ that
%	$ u_d( 0, x ) = f_{ 0, d }( x )$,
%	and which satisfy for all $ d \in \N $ 
%	that
%	$ u_d $ is a viscosity solution of
%	\begin{equation}
%	\begin{split}
%	( \tfrac{ \partial }{\partial t} u_d )( t, x ) 
%	& = 
%	( \tfrac{ \partial }{\partial x} u_d )( t, x )
%	\,
%	f_{ 1, d }( x )
%	+
%	\sum_{ i, j = 1 }^d
%	a_{ d, i, j }
%	\,
%	( \tfrac{ \partial^2 }{ \partial x_i \partial x_j } u_d )( t, x )
%	\end{split}
%	\end{equation}
%	for $ ( t, x ) \in (0,T) \times \R^d $.
%	This establishes item~\eqref{theoremDNNerrorEstimate:ItemExistence}. 
%	It thus remains to prove item~\eqref{theoremDNNerrorEstimate:Estimate}.
	Throughout this proof
		let $(\Phi_{d,N,M,\delta})_{d,N,M\in\N,\delta\in (0,1]}\subseteq \ANNs$, $\mathcal{C}_1,\allowbreak \mathfrak{C}\in (0,\infty)$ satisfy
		\begin{enumerate}[(I)]
			\item that for all 
			%$N\in\N\cap [T,\infty)$, $d,M\in\N$  
			$d,N,M\in\N$, $\delta\in (0,1]$
			it holds that $\functionANN(\Phi_{d,N,M,\delta})\in C(\R^{d+1},\R)$, and
			\begin{equation}\label{thmDNNerrorEstimate:BasisEstimate}
			\begin{split}
			& \left[
			\int_{[0,T]\times\R^d}
			\left\vert
			u_d(y) 
			- 
			\big[\functionANN(\Phi_{d,N,M,\delta})\big](y)
			\right\vert^p
			\,
			\nu_d (d y)
			\right]^{\!\nicefrac{1}{p}} 
			\\&\le
			\mathcal{C}_1 \left[\max\big\{1,\nu_d([0,T]\times\R^d)\big\}\right]^{\!\nicefrac{1}{p}}
			\\&\quad\cdot \left[ \frac{d^{\kappa(\kappa+4)+\max\{\eta,\kappa(2\kappa+1)\}}}{N^{1/2}}
			+ \frac{d^{\kappa+\max\{\eta,\kappa^2\}}}{M^{1/2}}
			+\delta {d}^{\nicefrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}+\eta} \right]
			\!
			\end{split}
			\end{equation}
			and
			\item \label{thmDNNerrorEstimate:itemParam}
			that for all 
			$d,N,M\in\N$, $\delta\in (0,1]$
			it holds that
			\begin{equation}
			\begin{split}
			&\paramANN(\Phi_{d,N,M,\delta})
			\le \mathfrak{C} M^2 d^{8\max\{2,\kappa\}}N^{5+4\kappa} (\max\{\log_2(\delta^{-1}),1\})^2
			\end{split}
			\end{equation}
		\end{enumerate}	
	(cf.\ Proposition~\ref{prop:DNNerrorEstimate}),
let	$\mathcal{C}_3,\mathcal{C}\in (0,\infty)$ be the real numbers which satisfy that
\begin{equation}\label{thmDNNerrorEstimate:thirdConstant}
\mathcal{C}_3=\max\!\left\{0,\log_2(3\,\mathcal{C}_1\,\eta)\right\}+\tfrac{1}{\log(2)}+\tfrac{1}{\log(2)}\,[\tfrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}+2\eta]
\end{equation}	
and
\begin{equation}\label{thmDNNerrorEstimate:totalConstant}
	\mathcal{C}=\mathfrak{C}\, 2^{7+4\kappa}\,  (3\mathcal{C}_1\eta)^{14+8\kappa} \,(\max\{\mathcal{C}_3,1\})^2,
\end{equation}
let $\mathcal{D}_{d,\varepsilon}\in (0,1]$, $d\in\N$, $\varepsilon\in (0,1]$, be the real numbers which satisfy for all $d\in\N$, $\varepsilon\in (0,1]$ that 
\begin{equation}\label{thmDNNerrorEstimate:ProductAccuracy}
	\mathcal{D}_{d,\varepsilon}=\min\!\left\{1,(3\mathcal{C}_1\eta)^{-1}\varepsilon d^{-\nicefrac{1}{2}(3\kappa+1)-2\kappa\max\{2\kappa,3\}-2\eta}\right\}\!,
\end{equation}
let $\mathfrak{M}_{d,\varepsilon}\in \N$, $d\in\N$, $\varepsilon\in (0,1]$, be the natural numbers which satisfy for all $d\in\N$, $\varepsilon\in (0,1]$ that 
\begin{equation}\label{thmDNNerrorEstimate:MCAccuracy}
\mathfrak{M}_{d,\varepsilon}=\min\!\left[\N\cap \!\big[(3\mathcal{C}_1\eta)^2 \varepsilon^{-2}d^{2\kappa+2\max\{\eta,\kappa^2\}+2\eta},\infty\big)\right]\!,
\end{equation}
let $\mathfrak{N}_{d,\varepsilon}\in \N$, $d\in\N$, $\varepsilon\in (0,1]$, be the natural numbers which satisfy for all $d\in\N$, $\varepsilon\in (0,1]$ that 
	\begin{equation}\label{thmDNNerrorEstimate:EulerAccuracy}
	\mathfrak{N}_{d,\varepsilon}=\min\!\left[\N\cap \!\big[(3\mathcal{C}_1\eta)^2 \varepsilon^{-2}d^{2\kappa(\kappa+4)+2\max\{\eta,\kappa(2\kappa+1)\}+2\eta},\infty\big)\right]\!,
	\end{equation}
	and let $(\Psi_{d,\varepsilon})_{d\in\N,\varepsilon\in (0,1]}\subseteq \ANNs$ satisfy for all 	$d\in\N,\varepsilon\in (0,1]$ that 
%	$
%	\Psi_{d,\varepsilon}=\Phi_{d,\mathfrak{N}_{d,\varepsilon},\mathfrak{M}_{d,\varepsilon},\mathcal{D}_{d,\varepsilon}}.
%	$
	\begin{equation}\label{thmDNNerrorEstimate:ChoiceANN}
	\Psi_{d,\varepsilon}=\Phi_{d,\mathfrak{N}_{d,\varepsilon},\mathfrak{M}_{d,\varepsilon},\mathcal{D}_{d,\varepsilon}}.
	\end{equation}	
Observe that \eqref{theoremDNNerrorEstimate:MeasureAssumption} and \eqref{thmDNNerrorEstimate:BasisEstimate} ensure that for all 
%$N\in\N\cap [T,\infty)$, $d,M\in\N$  
$d,N,M\in\N$, $\delta\in (0,1]$
it holds that 
\begin{equation}
\begin{split}
& \left[
\int_{[0,T]\times\R^d}
\left\vert
u_d(y) 
- 
\big[\functionANN(\Phi_{d,N,M,\delta})\big](y)
\right\vert^p
\,
\nu_d (d y)
\right]^{\!\nicefrac{1}{p}} 
\\&\le
\mathcal{C}_1 \left[\max\big\{1,\nu_d([0,T]\times\R^d)\big\}\right]^{\!\nicefrac{1}{p}}
\\&\quad\cdot \left[ \frac{d^{\kappa(\kappa+4)+\max\{\eta,\kappa(2\kappa+1)\}}}{N^{1/2}}
+ \frac{d^{\kappa+\max\{\eta,\kappa^2\}}}{M^{1/2}}
+\delta {d}^{\nicefrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}+\eta} \right]
\\&\le
\mathcal{C}_1 \eta
 \left[ \frac{d^{\kappa(\kappa+4)+\max\{\eta,\kappa(2\kappa+1)\}+\eta}}{N^{1/2}}
+ \frac{d^{\kappa+\max\{\eta,\kappa^2\}+\eta}}{M^{1/2}}
+\delta {d}^{\nicefrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}+2\eta} \right]
\!.
\end{split}
\end{equation}	
Combining this and \eqref{thmDNNerrorEstimate:ChoiceANN} with \eqref{thmDNNerrorEstimate:ProductAccuracy}, \eqref{thmDNNerrorEstimate:MCAccuracy}, and  \eqref{thmDNNerrorEstimate:EulerAccuracy} demonstrates that for all $d\in\N$, $\varepsilon\in (0,1]$ it holds that 
\begin{equation}\label{thmDNNerrorEstimate:errorFinal}
\begin{split}
& \left[
\int_{[0,T]\times\R^d}
\left\vert
u_d(y) 
- 
\big[\functionANN(\Psi_{d,\varepsilon})\big](y)
\right\vert^p
\,
\nu_d (d y)
\right]^{\!\nicefrac{1}{p}} 
\\&= \left[
\int_{[0,T]\times\R^d}
\left\vert
u_d(y) 
- 
\big[\functionANN(\Phi_{d,\mathfrak{N}_{d,\varepsilon},\mathfrak{M}_{d,\varepsilon},\mathcal{D}_{d,\varepsilon}})\big](y)
\right\vert^p
\,
\nu_d (d y)
\right]^{\!\nicefrac{1}{p}} 
\\&\le
\mathcal{C}_1 \eta
\left[ \frac{d^{\kappa(\kappa+4)+\max\{\eta,\kappa(2\kappa+1)\}+\eta}}{\vert\mathfrak{N}_{d,\varepsilon}\vert^{1/2}}
+ \frac{d^{\kappa+\max\{\eta,\kappa^2\}+\eta}}{\vert\mathfrak{M}_{d,\varepsilon}\vert^{1/2}}
+\mathcal{D}_{d,\varepsilon} {d}^{\nicefrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}+2\eta} \right]
\\&\le
\mathcal{C}_1 \eta
\bigg[ \frac{d^{\kappa(\kappa+4)+\max\{\eta,\kappa(2\kappa+1)\}+\eta}}{\left\vert(3\mathcal{C}_1\eta)^2 \varepsilon^{-2}d^{2\kappa(\kappa+4)+2\max\{\eta,\kappa(2\kappa+1)\}+2\eta}\right\vert^{1/2}}
+ \frac{d^{\kappa+\max\{\eta,\kappa^2\}+\eta}}{\left\vert(3\mathcal{C}_1\eta)^2 \varepsilon^{-2}d^{2\kappa+2\max\{\eta,\kappa^2\}+2\eta}\right\vert^{1/2}}
\\&\hspace{1.5cm}+(3\mathcal{C}_1\eta)^{-1}\varepsilon d^{-\nicefrac{1}{2}(3\kappa+1)-2\kappa\max\{2\kappa,3\}-2\eta} {d}^{\nicefrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}+2\eta} \bigg]
\\&=\mathcal{C}_1\eta \left(\frac{1}{3\mathcal{C}_1\eta \varepsilon^{-1}}+\frac{1}{3\mathcal{C}_1\eta \varepsilon^{-1}}+\frac{\varepsilon}{3\mathcal{C}_1\eta }\right)
=\varepsilon.
\end{split}
\end{equation}
In addition, observe that \eqref{thmDNNerrorEstimate:thirdConstant} and \eqref{thmDNNerrorEstimate:ProductAccuracy} demonstrate that for all $d\in\N$, $\varepsilon\in (0,1]$ it holds that
\begin{equation}
\begin{split}
&\log_2((\mathcal{D}_{d,\varepsilon})^{-1})
=\max\!\left\{0,\log_2\!\big(3\,\mathcal{C}_1\,\eta\,\varepsilon^{-1}\, d^{\nicefrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}+2\eta}\big)\right\}
\\&\le \max\!\left\{0,\log_2(3\,\mathcal{C}_1\,\eta)+\log_2(\varepsilon^{-1})+[\tfrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}+2\eta]\log_2(d)\right\}
\\&\le \max\!\left\{0,\log_2(3\,\mathcal{C}_1\,\eta)\right\}+\tfrac{1}{\log(2)}\, \varepsilon^{-1}+\tfrac{1}{\log(2)}\,[\tfrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}+2\eta]d
\\&\le  \varepsilon^{-1}d \big(\max\!\left\{0,\log_2(3\,\mathcal{C}_1\,\eta)\right\}+\tfrac{1}{\log(2)}+\tfrac{1}{\log(2)}\,[\tfrac{1}{2}(3\kappa+1)+2\kappa\max\{2\kappa,3\}+2\eta]\big)
\\&\le  \varepsilon^{-1}d\, \mathcal{C}_3.
\end{split}
\end{equation}	
Combining this with \eqref{thmDNNerrorEstimate:itemParam}, \eqref{thmDNNerrorEstimate:totalConstant}, \eqref{thmDNNerrorEstimate:MCAccuracy}, \eqref{thmDNNerrorEstimate:EulerAccuracy}, and \eqref{thmDNNerrorEstimate:ChoiceANN} proves that  for all $d\in\N$, $\varepsilon\in (0,1]$ it holds that
\begin{equation}
\begin{split}
\paramANN(\Psi_{d,\varepsilon})
&\le \mathfrak{C} (\mathfrak{M}_{d,\varepsilon})^2 d^{8\max\{2,\kappa\}}(\mathfrak{N}_{d,\varepsilon})^{5+4\kappa} (\max\{\log_2((\mathcal{D}_{d,\varepsilon})^{-1}),1\})^2
\\&\le \mathfrak{C} \big[(3\mathcal{C}_1\eta)^2 \varepsilon^{-2}d^{2\kappa+2\max\{\eta,\kappa^2\}+2\eta}+1\big]^{\!2} d^{8\max\{2,\kappa\}} (\max\{\varepsilon^{-1}d\, \mathcal{C}_3,1\})^2
\\&\quad\cdot\big[(3\mathcal{C}_1\eta)^2 \varepsilon^{-2}d^{2\kappa(\kappa+4)+2\max\{\eta,\kappa(2\kappa+1)\}+2\eta}+1\big]^{\!5+4\kappa} 
\\&\le \mathfrak{C} 2^{7+4\kappa} (3\mathcal{C}_1\eta)^4 \varepsilon^{-4}d^{4\kappa+4\max\{\eta,\kappa^2\}+4\eta} d^{8\max\{2,\kappa\}} \varepsilon^{-2}d^2 (\max\{\mathcal{C}_3,1\})^2
\\&\quad\cdot(3\mathcal{C}_1\eta)^{10+8\kappa} \varepsilon^{-10-8\kappa}d^{[2\kappa(\kappa+4)+2\max\{\eta,\kappa(2\kappa+1)\}+2\eta](5+4\kappa)} 
\\&\le \mathfrak{C} 2^{7+4\kappa}  \cdot(3\mathcal{C}_1\eta)^{14+8\kappa} \varepsilon^{-16-8\kappa} (\max\{\mathcal{C}_3,1\})^2
\\&\quad\cdot d^{2+4\kappa+4\max\{\eta,\kappa^2\}+4\eta+8\max\{2,\kappa\}+[2\kappa(\kappa+4)+2\max\{\eta,\kappa(2\kappa+1)\}+2\eta](5+4\kappa)}
\\&\le \mathcal{C} \varepsilon^{-16-8\kappa} 
d^{2+4\kappa+4\max\{\eta,\kappa^2\}+4\eta+8\max\{2,\kappa\}+[2\kappa(\kappa+4)+2\max\{\eta,\kappa(2\kappa+1)\}+2\eta](5+4\kappa)}.  
\end{split}
\end{equation}
This and \eqref{thmDNNerrorEstimate:errorFinal}	establish item~\eqref{theoremDNNerrorEstimate:Estimate} and item~\eqref{theoremDNNerrorEstimate:Param}.
	The proof of Theorem~\ref{theorem:DNNerrorEstimate} is thus completed.
\end{proof}

\begin{cor}
	\label{cor:DNNerrorEstimate}
	Let 
	$ T, \kappa \in (0,\infty) $, $\eta \in [1, \infty)$,  $p \in [2, \infty)$,
	assume for all $x\in \R$ that $\activation(x)=\max\{x,0\}$,
	let 
	$
	A_d = ( a_{ d, i, j } )_{ (i, j) \in \{ 1, \dots, d \}^2 } $ $ \in \R^{ d \times d }
	$,
	$ d \in \N $,
	be symmetric positive semidefinite matrices, 
	for every $ d \in \N $ 
	let 
	$
	\left\| \cdot \right\|_{ \R^d } \colon \R^d \to [0,\infty)
	$
	be the Euclidean norm on $\R^d$, let $\nu_d  \colon \mathcal{B}([0,T]\times\R^d) \to [0,\infty)$, $d\in\N$, be finite measures which satisfy for all $d\in\N$ that 
	%\begin{equation}
	%	\sup_{d \in \N} \left[ d^{-\theta p}
	%	\int_{\R^d}  
	%	\|{x}\|_{\R^d}^{ p \kappa } \,
	%	\nu_{ d } (dx)\right]
	%	< 
	%	\infty
	%	,
	%\end{equation}
	%$ 
	%\int_{\R^d}  
	%\|{x}\|_{\R^d}^{ p \kappa } \,
	%\nu_{ d } (dx)
	%\le \eta d^{\theta p}
	%,$
	\begin{equation}\label{corDNNerrorEstimate:MeasureAssumption}
	\left[\max\!\left\{1,\nu_d([0,T]\times\R^d),\int_{[0,T]\times \R^d} 
	\|x \|_{ \R^d }^{2p \max\{2\kappa, 3\}}
	\, \nu_d (d t, d x) \right\}\right]^{\!\nicefrac{1}{p}}\leq \eta d^{\eta},
	\end{equation}
	%$ \big(\textint_{[0,T]\times \R^d} 
	%\|z \|_{ \R^d }^{p \max\{2\kappa, \kappa+1\}}
	%\, \nu_d (d(s,z)) \big)^{\!\nicefrac{1}{p}}\leq \eta d^{\eta}$,
	%$ \big(\textint_{\R^d} 
	%\|z \|_{ \R^d }^{p (2\kappa+1)}
	%\, \nu_d (dz) \big)^{\!\nicefrac{1}{p}}\leq \eta d^{\eta}$,
	let
	$ f_{0,d} \colon \R^d \to \R $, $ d \in \N $,
	and
	$ f_{ 1, d } \colon \R^d \to \R^d $,
	$ d \in \N $,
	be functions,
	let 
	$
	( \phi^{ m, d }_{ \varepsilon } )_{ 
		(m, d, \varepsilon) \in \{ 0, 1 \} \times \N \times (0,1] 
	} 
	\subseteq \mathcal{N}
	$ satisfy for all
	$ d \in \N $, 
	$ \varepsilon \in (0,1] $
	that
	$
	\mathcal{R}( \phi^{ 0, d }_{ \varepsilon } )
	\in 
	C( \R^d, \R )
	$,
	$
	\mathcal{R}( \phi^{ 1, d }_{ \varepsilon } )
	\in
	C( \R^d, \R^d )
	$, and
	$\sum_{ m = 0 }^1
	\mathcal{P}( \phi^{ m, d }_{ \varepsilon } ) 
	\leq \kappa d^{ \kappa } \varepsilon^{ - \kappa }
	$,  
	assume for all
	$ d \in \N $, 
	$ \varepsilon \in (0,1] $, 
	$ 
	x, y \in \R^d
	$
	that 
	\begin{gather}
	\label{corDNNerrorEstimate:growthPhiOne}
	%	(\mathcal{R}\phi^{2,d})(x) = x, \qquad
	\|
	\big[\functionANN(\phi^{ 1, d }_{ \varepsilon })\big](x)    
	\|_{ \R^d }	
	\leq 
	\kappa ( d^{ \kappa } + \| x \|_{ \R^d } ),
	\\ \label{corDNNerrorEstimate:growthMatrix}
	|
	f_{ 0, d }( x )
	| 
	+
	\smallsum\nolimits_{ i , j = 1 }^d
	| a_{ d, i, j } |
	\leq 
	\kappa d^{ \kappa }
	( 1 + \| x \|^{ \kappa }_{ \R^d } )
	,
	\\
	\label{corDNNerrorEstimate:appr:coef}| 
	f_{ 0, d }(x) 
	- 
	\big[\functionANN(\phi^{ 0, d }_{ \varepsilon })\big] (x)
	|
	+
	\| 
	f_{ 1, d }(x) 
	- 
	\big[\functionANN(\phi^{ 1, d }_{ \varepsilon })\big] (x)
	\|_{ \R^d }
	\leq 
	\varepsilon \kappa d^{ \kappa }
	(
	1 + \| x \|^{ \kappa }_{ \R^d }
	),
	\\
	\label{corDNNerrorEstimate:approximationLocallyLipschitz}| \big[\functionANN(\phi^{ 0, d }_{ \varepsilon })\big] (x) - \big[\functionANN(\phi^{ 0, d }_{ \varepsilon })\big] (y)| \leq \kappa d^{\kappa} (1 + \|x\|_{\R^d}^{\kappa} + \|y \|_{\R^d}^{\kappa})\|x-y\|_{\R^d},
	\end{gather}
	%\begin{gather}
	%	\label{growthPhiOne}
	%%	(\mathcal{R}\phi^{2,d})(x) = x, \qquad
	%	\|
	%	\big[\functionANN(\phi^{ 1, d }_{ \varepsilon })\big](x)    
	%	\|_{ \R^d }	
	%	\leq 
	%	\kappa ( d^{ \kappa } + \| x \|_{ \R^d } ),
	%		\\
	%	\label{eq:appr:coef}| 
	%	f_{ 0, d }(x) 
	%	- 
	%	\big[\functionANN(\phi^{ 0, d }_{ \varepsilon })\big] (x)
	%	|
	%	+
	%	\| 
	%	f_{ 1, d }(x) 
	%	- 
	%	\big[\functionANN(\phi^{ 1, d }_{ \varepsilon })\big] (x)
	%	\|_{ \R^d }
	%	\leq 
	%	\varepsilon \kappa d^{ \kappa }
	%	(
	%	1 + \| x \|^{ \kappa }_{ \R^d }
	%	),
	%	\\
	%	\label{approximationLocallyLipschitz}| \big[\functionANN(\phi^{ 0, d }_{ \varepsilon })\big] (x) - \big[\functionANN(\phi^{ 0, d }_{ \varepsilon })\big] (y)| \leq \kappa d^{\kappa} (1 + \|x\|_{\R^d}^{\kappa} + \|y \|_{\R^d}^{\kappa})\|x-y\|_{\R^d},
	%	\\ \label{growthMatrix}
	%		|
	%	f_{ 0, d }( x )
	%	| 
	%	+
	%	\smallsum\nolimits_{ i , j = 1 }^d
	%	| a_{ d, i, j } |
	%	\leq 
	%	\kappa d^{ \kappa }
	%	( 1 + \| x \|^{ \kappa }_{ \R^d } )
	%	,
	%\end{gather}
	and $\| 
	f_{ 1, d }( x ) 
	- 
	f_{ 1, d }( y )
	\|_{ \R^d }
	\leq 
	\kappa 
	\| x - y \|_{ \R^d }$, 
	and let $ u_d \colon [0,T] \times \R^{d} \to \R $,
	$ d \in \N $, be the unique continuous functions which satisfy for all $d \in \N$ that
	$
	\inf_{q \in (0,\infty)} \allowbreak
	\sup_{(t, x) \in [0, T] \times \R^d} \allowbreak
	\frac{ | u_d(t, x) | }{ 1 + \norm{x}_{\R^d}^q }
	\allowbreak<
	\infty
	$,
	which satisfy
	for all $ d \in \N $, $ x \in \R^d $ that
	$ u_d( 0, x ) = f_{ 0, d }( x )$,
	and which satisfy for all $ d \in \N $ 
	that
	$ u_d $ is a viscosity solution of
	\begin{equation}
	\begin{split}
	( \tfrac{ \partial }{\partial t} u_d )( t, x ) 
	& = 
	( \tfrac{ \partial }{\partial x} u_d )( t, x )
	\,
	f_{ 1, d }( x )
	+
	\sum_{ i, j = 1 }^d
	a_{ d, i, j }
	\,
	( \tfrac{ \partial^2 }{ \partial x_i \partial x_j } u_d )( t, x )
	\end{split}
	\end{equation}
	for $ ( t, x ) \in (0,T) \times \R^d $ (cf.\ Theorem~\ref{thm:feynman}).
	Then there exist $\mathfrak{C}\in (0,\infty)$ and $(\Psi_{d,\varepsilon})_{d\in\N,\varepsilon\in (0,1]}\subseteq \ANNs$ which satisfy
		that for all 
		%$N\in\N\cap [T,\infty)$, $d,M\in\N$  
		$d\in\N$, $\varepsilon\in (0,1]$
		it holds that $\paramANN(\Psi_{d,\varepsilon})
		\le \mathfrak{C} \varepsilon^{-\mathfrak{C}}  d^{\mathfrak{C}}$, $\functionANN(\Psi_{d,\varepsilon})\in C(\R^{d+1},\R)$, and
		\begin{equation}
		\begin{split}
		& \left[
		\int_{[0,T]\times\R^d}
		\left\vert
		u_d(y) 
		- 
		\big[\functionANN(\Psi_{d,\varepsilon})\big](y)
		\right\vert^p
		\,
		\nu_d (d y)
		\right]^{\!\nicefrac{1}{p}} 
		\le
		\varepsilon.
		\end{split}
		\end{equation}
\end{cor}

\begin{proof}[Proof of Corollary~\ref{cor:DNNerrorEstimate}]
	Throughout this proof 
let $\mathcal{C}\in (0,\infty)$ and $(\Psi_{d,\varepsilon})_{d\in\N,\varepsilon\in (0,1]}\subseteq \ANNs$ satisfy
\begin{enumerate}[(I)]
	\item
	\label{corDNNerrorEstimate:Estimate}
	that for all 
	%$N\in\N\cap [T,\infty)$, $d,M\in\N$  
	$d\in\N$, $\varepsilon\in (0,1]$
	it holds that $\functionANN(\Psi_{d,\varepsilon})\in C(\R^{d+1},\R)$ and
	\begin{equation}
	\begin{split}
	& \left[
	\int_{[0,T]\times\R^d}
	\left\vert
	u_d(y) 
	- 
	\big[\functionANN(\Psi_{d,\varepsilon})\big](y)
	\right\vert^p
	\,
	\nu_d (d y)
	\right]^{\!\nicefrac{1}{p}} 
	\le
	\varepsilon
	\end{split}
	\end{equation}
	and
	\item \label{corDNNerrorEstimate:Param}
	that for all 
	$d\in\N$, $\varepsilon\in (0,1]$
	it holds that
	\begin{equation}
	\begin{split}
	&\paramANN(\Psi_{d,\varepsilon})
	\\&\le \mathcal{C} \varepsilon^{-16-8\kappa}  d^{2+4\kappa+4\max\{\eta,\kappa^2\}+4\eta+8\max\{2,\kappa\}+[2\kappa(\kappa+4)+2\max\{\eta,\kappa(2\kappa+1)\}+2\eta](5+4\kappa)} 
	\end{split}
	\end{equation}
\end{enumerate}
(cf.\ Theorem~\ref{theorem:DNNerrorEstimate})	
	and let $\mathfrak{C}\in (0,\infty)$ be the real number which satisfies that 
\begin{multline}\label{corDNNerrorEstimate:finalConstant}
	\mathfrak{C}=\max\!\big\{\mathcal{C}, 16+8\kappa,  2+4\kappa+4\max\{\eta,\kappa^2\}+4\eta+8\max\{2,\kappa\}\\+[2\kappa(\kappa+4)+2\max\{\eta,\kappa(2\kappa+1)\}+2\eta](5+4\kappa)\big\}.
\end{multline}
Observe that \eqref{corDNNerrorEstimate:Param} and \eqref{corDNNerrorEstimate:finalConstant} show that for all 
$d\in\N$, $\varepsilon\in (0,1]$
it holds that
\begin{equation}
\begin{split}
&\paramANN(\Psi_{d,\varepsilon})
\\&\le \mathcal{C} \varepsilon^{-16-8\kappa}  d^{2+4\kappa+4\max\{\eta,\kappa^2\}+4\eta+8\max\{2,\kappa\}+[2\kappa(\kappa+4)+2\max\{\eta,\kappa(2\kappa+1)\}+2\eta](5+4\kappa)} 
\\&\le \mathfrak{C} \varepsilon^{-\mathfrak{C}}  d^{\mathfrak{C}}.
\end{split}
\end{equation}
	This and \eqref{corDNNerrorEstimate:Estimate}	complete
	the proof of Corollary~\ref{theorem:DNNerrorEstimate}.
\end{proof}


